Multivariate Rational Approximation

We present two approaches for computing rational approximations to multivariate functions, motivated by their effectiveness as surrogate models for high-energy physics (HEP) applications. Our first approach builds on the Stieltjes process to efficiently and robustly compute the coefficients of the rational approximation. Our second approach is based on an optimization formulation that allows us to include structural constraints on the rational approximation, resulting in a semi-infinite optimization problem that we solve using an outer approximation approach. We present results for synthetic and real-life HEP data, and we compare the approximation quality of our approaches with that of traditional polynomial approximations.

==> apps_sm.tex <==
\clearpage
\section{Rational Approximation for HEP Experiment}\label{SEC:HEP}
Physics simulation programs are used to make predictions of known or
proposed phenomenon that can be compared to experiments.
Typically, the physics models inside the simulation contain a large number of parameters.
Some of these have a fundamental physical meaning, such as masses and
coupling strengths.    Others are purely pragmatic and compound imperfect knowledge about certain aspects of the model.  Both types of parameters are needed to make accurate predictions.

A typical problem in particle physics is to infer 
%\emph{unobservable} 
values, or ranges of values, for the model parameters by comparing experimentally observed data with
equivalent quantities obtained from simulations of physics processes.
In our example, the simulation predicts how postulated dark matter particles
interact with a Xenon-based detector in a process called ``direct
detection''.   In practice, the simulation predicts a number of signal
counts in the detector with certain characteristics.     
If the characteristic is a continuous variable, it is sometimes
divided up into a finite number of bins $b$.
The signal
model is specified by three parameters $p = \{m_\chi, c_{+}, c_{\pi}\}$,
where $m_\chi$ is the mass of the dark matter candidate particle and
$c_{+}, c_{\pi}$ are coupling strengths for the interaction of the
dark matter with the ordinary matter in the detector.   The case $c_+
= c_\pi = 0$ corresponds to no dark matter signal.   Even in the
absence of a signal, counts are observed in the detector from backgrounds.
The number of counts in a given bin $b$ is expected to follow a
Poisson distribution with a mean value determined from the simulation
assuming no signal.   After data $d$ has been collected, an analysis is
performed to determine which values of $p$ are compatible or excluded.   The
statistic called Likelihood, $\mathcal{L}(p|d)$, is constructed and
maximized to answer
this question:
\begin{equation}\label{eq:alikelihood}
    \mathcal{L}(p|d) = \prod\limits_b \frac{N_b(p) d_b e^{N_b(p)}}{\Gamma(d_b+1)},
\end{equation}
where the product runs over all bins $b$, the numbers $d_b$ are
the experimentally measured quantities for each bin, and  $N_b(p)$ 
is the number of total counts in the bin $b$ predicted by the
parameters $p$, which range over a set of $k$ individual values $p^{(k)}$.

The calculation of $N_b(p^{(k)})$ is computationally expensive and can
only be performed at a finite number of points $p^{(k)}$.
Fortunately, the predictions are smooth and can be represented by a
surrogate function $r_b(p)$ constructed from a finite number of
calculations $N_b(p^{(k)})$.   Here, we demonstrate the utility of the
rational approximation methods in performing an accurate analysis of
the data in comparison to brute force and other approximation methods.   
Instead of maximizing the  likelihood in \cref{eq:likelihood}, we maximize an approximate likelihood:
\begin{equation}\label{eq:alikelihood-app}
    \mathcal{L}(x|d) \approx \mathcal{\tilde{L}}(x|d) = \prod\limits_b \frac{r_b(x) d_b e^{r_b(x)}}{\Gamma(d_b+1)}.
\end{equation}
The maximization of the likelihood itself is performed using 
the numerical tool MultiNest~\cite{Feroz:2008xx,Feroz:2013hea,pymultinest}.
 The data are simulated using a specific framework
of the generalized spin-independent response to dark matter in direct detection
experiments~\cite{Hoferichter:2016nvd}.
The $d_b$ used in
\cref{eq:likelihood,eq:likelihood-app} are 
 $d_b$ = \{ 70.4 , 26.7 , 9.8 , 3.4 , 1.0 , 0.2 \} for $b=6$ bins.
Note that we fit a separate rational approximation for each bin $b$.   




% \begin{figure}[htb!]
%     \centering
%     \includegraphics[width=.68\textwidth]{images/expsetup.pdf}
%     \caption{\textcolor{blue}{Into supplement: Illustration of a typical problem setup in particle physics. Shown are
%         histogram skylines of observable experimental data (black) with observable
%         predictions coming from simulations at different points $x^{(k)}$ in the same parameter space (blue and red).
%         Numerical comparisons of the experimental with the simulated quantities are typically used to infer quantitative
%         statements on the (unobservable) parameters of the simulation. In this
%         example, one would e.g. be interested in finding parameter points $x$ such that the corresponding simulation
%        prediction resembles the experimental observation.}}
%     \label{fig:hepexample}
% \end{figure}

Our study consists of four separate analyses.    The first, or brute
force, analysis relies on the evaluation of $N_b(p^{(k)})$ over a dense set of 
parameter points $p^{(k)}$.   The second analysis uses a rational
approximation $r_b(p)$ based on far fewer parameter points.    A third
analysis is similar to the second, but demonstrates the effect of
poles.   The final analysis is based on a purely polynomial
approximation, similar to a previous study \cite{Cerdeno:2018bty}.
Our results are presented as 
two-dimensional projections of the 3-dimensional likelihood
called profile-likelihoods, which are quantities
normalised to the maximum observer likelihood.
These are produced using the tool superplot~\cite{Fowlie:2016hew}.
We have chose to show limits on the coupling strengths $c_+, c_\pi$
for a fixed value of $m_\chi$ \textcolor{blue}{(is the true?  if so, which value?).}

The results are summarized in Figure \cref{fig:nest-si-full} (fix this).
The darker regions in the plots represent a higher likelihood, or a
higher probability that the corresponding values of $c_+,c_\pi$ are
allowed by the data.
The top-left plot (\cref{fig:nest-si-full}) shows the projection of the likelihood obtained 
with  the full simulation \cref{eq:likelihood}.   
This is our ground truth for evaluating the approximation methods.
Qualitatively, we observe two ridges of equal likelihood in this
projection, showing that the allowed values of $c_+$ and $c_\pi$ are
highly correlated.   The top-right plot shows similar results using
the pole-free rational approximation, which is in good agreement with the ground truth both qualitatively
and quantitatively.   \textcolor{blue}{Is there a quantitative measure
  of the agreement between the projections?}
The bottom-left plot are the results using \cref{LinAlg},
which is less accurate due to spurious poles in the relevant parameter
domain.  Qualitatively, we find strong similarities with the ground truth, but the poles in some of the
$r_b(x)$ lead to a complete distortion of the evaluated likelihoods, and
therefore to a quantitatively wrong interpretation of the resulting plot as we
no longer find the dark region of equal likelihood present in
\cref{fig:nest-si-full,fig:nest-si-sip}.    Finally, the bottom-right
plot shows results using a polynomial approximation of order 7 (such that the number of coefficients is comparable to 
the number of coefficients used in the  rational approximations).  
The resulting likelihood projection \cref{fig:nest-si-poly} shows the
benefit of using rational approximations over polynomial ones; in this example,  the
polynomial approximations are  not able to capture the true likelihood
at all. 
Thus, the parameters inferred using the polynomial approximation would be misleading. 

The benefit of the rational approximation in our results is not simply
the agreement with the full simulation, but the relative computational
cost, summarized in \cref{tab:atimeloli}.
The algorithm terminates after about 30.000 evaluations of either $\mathcal{L}$ or the rational approximation
based $\tilde{\mathcal{L}}$. The difference in run-times is about a
factor of 50 to obtain similar results.   The number of parameters
considered in our case is modest, and we expect a significant speed-up
for likelihood evaluations using rational approximations for more
complex models.

\begin{table}
    \centering
    \begin{tabular}{l|c c}
        & Likelihood evaluations & total run-time~[s] \\ \hline
      using full simulation \cref{fig:nest-si-full} & 29459 & 14594 \\
    using $r_b$ with \cref{A:Polyak} & 29612 & 288
    \end{tabular}
    \caption{Summary of computational costs.}
    \label{tab:atimeloli}
\end{table}



% \begin{figure}[htb!]
%     \centering
%     \begin{subfigure}[b]{0.475\textwidth}
%         \centering
%         \includegraphics[width=.9\textwidth]{plots/multinest_SI/hard_2k/plot_2_3_profile_xlabel1_ylabel1.pdf}
%         \caption%
%         {{\small Result with full simulation}}    
%         \label{fig:nest-si-full}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.475\textwidth}  
%         \centering 
%         \includegraphics[width=.9\textwidth]{plots/multinest_SI/FNalsip44_2k/plot_2_3_profile_xlabel1_ylabel1.pdf}
%         \caption[]%
%         {{\small Result with pole-free rational approximation}}    
%         \label{fig:nest-si-sip}
%     \end{subfigure}
%     \vskip\baselineskip
%     \begin{subfigure}[b]{0.475\textwidth}   
%         \centering 
%         \includegraphics[width=.9\textwidth]{plots/multinest_SI/FNalla54_s1_2k//plot_2_3_profile_xlabel1_ylabel1.pdf}
%         \caption[]%
%         {{\small Result with non-pole-free rational approximation}}
%         \label{fig:nest-si-la}
%     \end{subfigure}
%     \quad
%     \begin{subfigure}[b]{0.475\textwidth}   
%         \centering 
%         \includegraphics[width=.9\textwidth]{plots/multinest_SI/p6_n/plot_2_3_profile_xlabel1_ylabel1.pdf}
%         \caption[]%
%         {{\small Result with polynomial approximation}}    
%         \label{fig:nest-si-poly}
%     \end{subfigure}
%     \caption[]
%     {\textcolor{blue}{add color bar} Two-dimensional profile-likelihood projections of a 3-dimensional
%         parameter space. The color-coding is such that regions of higher likelihood appear darker. The data is normalized to the maximum likelihood observed before plotting. We compare the result obtained with the full physics
% simulation output (\cref{fig:nest-si-full}) to the result obtained when using 
% pole-free rational approximations calculated with the semi-infinite approach (\cref{fig:nest-si-sip}).
% \cref{fig:nest-si-la} shows the effect of poles in the relevant parameter domain. The poles
% are visible as dark dots. For completeness, \cref{fig:nest-si-poly} shows the result when using
% polynomial approximations with a similar number of coefficients as in \cref{fig:nest-si-sip}.}
% \label{fig:nest-si}
% \end{figure}



==> errorData.tex <==
\ref{fn:f1}&9.405E+01&2.396E+01&1.580E+00&5.714E-01&1.511E+00&5.454E-01\\\hline
\ref{fn:f2}&3.986E+01&1.802E+01&1.158E+00&3.960E-01&1.163E+00&4.064E-01\\\hline
\ref{fn:f3}&9.526E+01&5.298E+01&1.530E-01&3.413E-02&1.815E-01&1.710E-02\\\hline
\ref{fn:f4}&1.302E-08&1.860E-09&5.474E-09&6.007E-10&5.528E-09&5.676E-10\\\hline
\ref{fn:f5}&5.865E+00&1.536E+00&1.320E+01&1.647E+01&1.362E+00&2.862E-01\\\hline
\ref{fn:f7}&3.540E-01&1.437E-01&1.354E-13&4.170E-14&4.054E-04&4.124E-04\\\hline
\ref{fn:f8}&2.063E+03&1.004E+03&3.536E-11&9.494E-12&1.239E-07&1.679E-07\\\hline
\ref{fn:f9}&9.575E+03&2.954E+03&2.533E-10&1.180E-10&9.033E-06&8.316E-06\\\hline
\ref{fn:f10}&2.627E+02&3.669E+01&1.261E-12&3.240E-13&3.177E-10&1.577E-10\\\hline
\ref{fn:f12}&3.165E+00&1.010E+00&3.797E-14&1.139E-14&4.531E-12&4.612E-12\\\hline
\ref{fn:f13}&3.638E-01&4.548E-02&2.092E-14&1.757E-15&2.124E-12&3.972E-13\\\hline
\ref{fn:f14}&1.422E+01&3.354E+00&2.393E-13&5.244E-14&1.018E-09&6.570E-10\\\hline
\ref{fn:f15}&1.056E+01&2.455E+00&1.386E-13&5.697E-14&2.025E-10&1.392E-10\\\hline
\ref{fn:f16}&5.729E+00&1.103E+00&6.223E-14&9.326E-15&1.214E-10&6.117E-11\\\hline
\ref{fn:f17}&6.923E+05&4.647E+05&1.156E+01&5.668E+00&1.157E+01&5.676E+00\\\hline
\ref{fn:f18}&2.625E+03&3.746E+02&3.496E+04&2.538E+04&1.636E+03&2.502E+02\\\hline
\ref{fn:f19}&9.950E-01&6.260E-02&2.126E-01&2.411E-02&2.104E-01&2.291E-02\\\hline
\ref{fn:f20}&1.467E+00&3.192E-01&1.181E+00&9.413E-02&1.136E+00&5.577E-03\\\hline
\ref{fn:f21}&9.957E+01&9.873E+01&3.672E+00&2.000E+00&4.864E+00&3.685E+00\\\hline
\ref{fn:f22}&3.252E-13&8.129E-14&1.980E-13&4.254E-14&8.653E-13&7.910E-13\\\hline

\ref{fn:f1}&7.748E+02&2.110E+02&3.250E+02&1.789E+02&2.027E+02&7.597E+00\\\hline
\ref{fn:f2}&3.259E+01&1.014E+01&1.462E+01&5.030E+00&1.483E+01&5.752E+00\\\hline
\ref{fn:f3}&1.548E+02&3.123E+01&1.280E+04&1.352E+04&3.845E+01&1.326E+00\\\hline
\ref{fn:f4}&3.343E+01&1.743E+01&6.086E+03&6.879E+03&1.341E+01&4.151E+00\\\hline
\ref{fn:f5}&8.997E+01&2.657E+01&2.029E+04&3.133E+04&4.541E+01&1.064E+01\\\hline
\ref{fn:f7}&3.674E+01&2.108E+01&1.616E+04&1.729E+04&1.426E+01&4.772E+00\\\hline
\ref{fn:f8}&1.936E+03&7.975E+02&3.046E+04&5.660E+04&5.106E+02&3.518E+02\\\hline
\ref{fn:f9}&9.465E+03&3.204E+03&1.986E+05&1.876E+05&1.432E+03&3.862E+02\\\hline
\ref{fn:f10}&7.710E+01&2.055E+01&4.158E+04&3.524E+04&6.078E+01&7.837E+00\\\hline
\ref{fn:f12}&1.158E+01&3.494E+00&1.082E+03&1.513E+03&9.140E+00&2.754E+00\\\hline
\ref{fn:f13}&5.823E+00&1.781E+00&6.132E+00&3.632E+00&3.892E+00&7.329E-01\\\hline
\ref{fn:f14}&6.619E+01&3.140E+01&1.405E+01&4.348E+00&1.356E+01&4.466E+00\\\hline
\ref{fn:f15}&1.855E+01&6.435E+00&3.947E+03&3.367E+03&1.154E+01&3.049E+00\\\hline
\ref{fn:f16}&5.062E+01&1.397E+01&2.611E+01&5.448E+00&3.020E+01&8.125E+00\\\hline
\ref{fn:f17}&6.721E+09&5.676E+09&2.212E+01&1.479E+01&1.198E+01&5.490E+00\\\hline
\ref{fn:f18}&2.694E+03&4.369E+02&1.092E+05&4.519E+04&1.951E+03&3.798E+02\\\hline
\ref{fn:f19}&2.104E+01&3.315E+00&4.014E+03&1.502E+03&1.564E+01&1.152E+00\\\hline
\ref{fn:f20}&1.462E+00&3.122E-01&1.139E+00&1.392E-02&1.136E+00&5.542E-03\\\hline
\ref{fn:f21}&4.440E+02&2.378E+02&2.339E+04&1.120E+04&4.047E+02&1.431E+02\\\hline
\ref{fn:f22}&6.646E+01&3.126E+01&4.716E+01&1.469E+01&3.189E+01&7.143E+00\\\hline

\ref{fn:f1}&2.268E+02&4.055E+01&4.906E+01&1.148E+01&4.681E+01&1.024E+01\\\hline
\ref{fn:f2}&9.191E+00&1.040E+00&1.307E+00&2.598E-01&1.233E+00&2.701E-01\\\hline
\ref{fn:f3}&1.297E+02&3.065E+01&1.314E+03&1.628E+03&2.252E+00&5.186E-01\\\hline
\ref{fn:f4}&3.343E-01&1.742E-01&1.014E+02&1.797E+02&1.445E-01&5.010E-02\\\hline
\ref{fn:f5}&3.977E+01&1.745E+01&4.554E+01&4.826E+01&3.136E+01&2.491E+01\\\hline
\ref{fn:f7}&7.831E-01&5.046E-01&3.224E+01&4.045E+01&3.823E-01&2.254E-01\\\hline
\ref{fn:f8}&2.510E+03&4.082E+02&2.796E+00&1.434E+00&2.780E+00&1.422E+00\\\hline
\ref{fn:f9}&1.544E+04&3.118E+03&1.767E+03&3.522E+02&1.559E+03&3.393E+02\\\hline
\ref{fn:f10}&2.631E+02&3.674E+01&9.992E-01&3.136E-01&9.973E-01&3.121E-01\\\hline
\ref{fn:f12}&3.137E+00&9.686E-01&9.244E-02&2.784E-02&9.170E-02&2.700E-02\\\hline
\ref{fn:f13}&2.648E+00&4.414E-01&1.912E+03&1.696E+03&1.599E+01&2.612E-01\\\hline
\ref{fn:f14}&4.884E+01&9.042E+00&2.239E+01&4.578E+00&2.187E+01&3.881E+00\\\hline
\ref{fn:f15}&1.051E+01&2.413E+00&1.686E-01&7.118E-02&1.663E-01&7.032E-02\\\hline
\ref{fn:f16}&1.202E+01&3.314E+00&5.122E+00&7.102E+00&1.730E+00&4.475E-01\\\hline
\ref{fn:f17}&6.940E+05&4.647E+05&1.171E+01&5.754E+00&1.174E+01&5.774E+00\\\hline
\ref{fn:f18}&2.624E+03&3.750E+02&6.229E+04&5.762E+04&1.713E+03&2.606E+02\\\hline
\ref{fn:f19}&3.343E+00&1.753E-01&3.223E+00&3.230E-01&3.098E+00&2.335E-01\\\hline
\ref{fn:f20}&1.466E+00&3.191E-01&1.132E+00&2.527E-03&1.136E+00&6.115E-03\\\hline
\ref{fn:f21}&4.869E+02&3.525E+02&7.654E+05&1.402E+06&2.304E+02&6.474E+01\\\hline
\ref{fn:f22}&6.646E-01&3.126E-01&4.219E-01&1.298E-01&4.135E-01&1.237E-01\\\hline


==> ideas.tex <==
\section{Rational Approximation}\label{sec:ideas}

We start by recapping one-dimensional Rational approximation, and then show that it naturally generalizes to multiple dimensions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Basic Notation for Rational Approximation}

\sven{Use "mathy" notation?} PROFESSOR (and POUNDERs) use polynomial basis functions. However, in some applications, it
may be more appropriate to use (multi-variate) rational approximations (e.g. Leonard-Jones
potential). Thus, we want to approximate 
\[ f_b(\p) = \frac{g_b(\p)}{h_b(\p)} ,\]
where $g_b(\p)$ and $h_b(\p)$ are multi-dimensional polynomials of fixed degree.

This approach creates a number of challenges:
\begin{enumerate}
  \item Naive fitting polynomials of $g_b(\p)$ and $h_b(\p)$ results in a nonlinear least-squares
    problem:
    \begin{equation}\label{eq:PadeLS}
      \mini_{g_b,h_b} \; \sum_i \left( v_b^{(i)} - \frac{g_b(\p^{(i)})}{h_b(\p^{(i)})} \right)^2,
    \end{equation}
    where we minimize over the coefficients of the polynomials, $g_b, h_b$.
  \item Handling of $h_b(\p) \not = 0$ is challenging, because it creates an open set
    over which we optimize, but this may not be an issue, if we assume that all values are
    finite, i.e. $| v_b^{(i)} | < \infty$.
  \item In practice, we expect the denominator to be non-zero in the region of interest, i.e.
    we assume wlog that
    \[ h_b(\p) \geq 1 \quad \forall \p \in [l,u], \]
    which is a semi-infinite constraint.
\end{enumerate}
We will assume wlog that $\text{MC}_b(\p^{(i)}) =: v_b^{(i)}$ is finite, i.e. $| v_b^{(i)} | < \infty$
(otherwise, we gain information about a pole, and re-evaluate $\text{MC}_b()$ at a nearby point).

The first observation is that we can linearize the least-squares fitting problem by multiplying through
by $h_b(\p^{(i)})$,
provided that $h_b(\p^{(i)}) \not = 0$, which follows from our assumption that $| v_b^{(i)} | < \infty$,
resulting in the {\em linear} least-squares problem
\[ \mini_{g_b,h_b} \; \sum_i \left( h_b(\p^{(i)}) v_b^{(i)} - g_b(\p^{(i)}) \right)^2 .\]
However, this multiplication also creates a trivial solution to our least-squares problem,
which is $h_b(\p) = g_b(\p) = 0$. We show in the next two sections how to overcome this issue
(first in the well-established one-dimensional case then for the multi-dimensional extension).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{One-Dimensional Rational Approximations}

\sven{delete this section?}
We are interested in deriving a rational approximation:
\begin{equation}\label{eq:PadeOneD}
  f : \R \to \R, \quad f(p) \simeq \frac{h(p)}{g(p)}
\end{equation}
by fitting the coefficients of $h(p), g(p)$ to data, $(p_l, f(p_l)$. Denoting the polynomials
as
\begin{equation}
  h(p) = a_0 + a_1 p + a_2 p^2 + \ldots + a_m p^m \quad \text{and} \quad
  g(p) = b_0 + b_1 p + b_2 p^2 + \ldots + b_n p^n,
\end{equation}
we observe that we have $K=(m+1)+(n+1)-1$ degrees of freedom (one less, because we can scale
either $a_0=1$ or $b_0=1$ wlog). Assuming that we have $K$ data points, $\left(p_l, f(p_l)\right), l=1,\ldots,K$
that are ``nicely'' chosen, the fitting problem can be written as
\begin{equation}\label{eq:FitPadeOneD}
  f(p_l) =  \frac{h(p_l)}{g(p_l)} \quad \Leftrightarrow \quad g(p_l)f(p_l) =  h(p_l) \quad \forall l=1,\ldots,K
\end{equation}
provided that $g(p_l) \not = 0$. We note, that \eqref{eq:FitPadeOneD} is a square linear
system of equations in $K$ unknowns. To solve this system, we provisionally add coefficients
up to order $K$ to $h(p)$ and $g(p)$ (which we will enforce to be zero later). Thus, we write
the polynomials as
\begin{equation}
  \begin{array}{rcl}
    h(p) & = & a_0 + a_1 p + a_2 p^2 + \ldots + a_m p^m + \ldots + a_K p^K \\
    \text{and} & & \\
    g(p) & = & b_0 + b_1 p + b_2 p^2 + \ldots + b_n p^n + \ldots + b_K p^K.
  \end{array}
\end{equation}
We let the Vandermonde matrix of order $K$ be
\begin{equation}
  V := \left[ \begin{array}{ccccc}
      1 & p_1 & p_1^2 & \ldots & p_1^K \\
        &     &      &        &       \\
      \vdots & \vdots & \vdots &   & \vdots \\
        &     &      &        &       \\
      1 & p_K & p_K^2 & \ldots & p_K^K 
       \end{array}\right]
\end{equation}
and we define the diagonal matrix $F := \text{diag}(f(p_1), \ldots, f(x_K))$, and
vectors of coefficients $a=(a_0,\ldots,a_K)^T$ and $b=(b_0,\ldots,b_K)^T$. Then,
we can write \eqref{eq:FitPadeOneD} compactly as
\[ F V b = V a . \]
If we assume that $V$ is invertible (which imposes a condition on the interpolation points),
then we can rewrite this system as
\[ a = V^{-1} F V b =: Z b , \]
where $Z = V^{-1} F V$. Now recall, that $b_{n+1} = \ldots = b_K = 0$, and denote the first
$n$ components of $b$ by $\hat{b}$, and similarly define $\hat{Z} := Z[:,1:n]$ using Matlab/Python
notation. Then it follows that
\[ a = \hat{Z} \hat{b} ,\]
which is a ``skinny'' system of equations. If we also enforce the condition that
$a_{m+1} = \ldots = a_K = 0$, then we can write this system as
\[ \left(\begin{array}{c}
     a_0 \\ \vdots \\ a_m \\ \hline a_{m+1} \\ \vdots \\ a_K
   \end{array}\right)
   =
   \left[\begin{array}{c} \\ \bar{Z} \\ \\ \hline \\ \tilde{Z} \\ \phantom{+} \end{array}\right]
   \left(\begin{array}{c}
     b_0 \\ \vdots \\ b_n
   \end{array}\right)
   \quad \text{or}\quad \hat{a} = \bar{Z} \hat{b}, \quad \text{and} \quad 0 = \tilde{Z} \hat{b}
\]
We now observe that the last set of equations, $0 = \tilde{Z} \hat{b}$, has $K-m-1=m+n+1-m-1=n$ equations
an $n+1$ unknowns. Thus, if the equations are consistent, we can choose $\hat{b}$ to be a vector that
lies in the null-space of $\tilde{Z}$. Forming an SVD of $\tilde{Z}$ (another $V$ here ;-)
\[ \tilde{Z} = \tilde{U} \tilde{\Sigma} \tilde{V}^T ,\]
we choose $\hat{b} := \tilde{V}[:,n+1]$ as the last singular vector, then obtain $\hat{a} = \bar{Z} \hat{b}$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Multi-Dimensional Rational Approximations}

\sven{Rewrite?}
The generalization to multi-dimensional  rational approximation follows the same ideas as the one-dimensional
case. We start by considering the $N$ dimensional polynomials:
\begin{equation}
  h(p) = a^{(0)} + \sum_{i=1}^N a^{(1)}_{i} p_i + \sum_{i_1,i_2=1}^N a^{(2)}_{i_1,i_2} p_{i_1} p_{i_2}
     + \ldots + \sum_{i_1,\ldots,i_m=1}^N a^{(m)}_{i_1,\ldots,i_m} p_{i_1} \cdots p_{i_m} 
\end{equation}
and
\begin{equation}
  g(p) = b^{(0)} + \sum_{i=1}^N b^{(1)}_{i} p_i + \sum_{i_1,i_2=1}^N b^{(2)}_{i_1,i_2} p_{i_1} p_{i_2}
     + \ldots + \sum_{i_1,\ldots,i_n=1}^N b^{(n)}_{i_1,\ldots,i_n} p_{i_1} \cdots p_{i_n} .
\end{equation}
We let $C_n^{(N)}$ be the number of coefficients of an $n^{th}$ degree polynomial in $P$ variables,
then it can be shown that
\[ C_n^{(N)} = 1 + \sum_{i=1}^n \frac{1}{i!} \prod_{j=0}^{i-1} (P + j) ,\]
and we have $K= C_m^{(N)} + C_n^{(N)} - 1$ degrees of freedom in our interpolation problem.

\paragraph{Outline of Remainder of Section.} 
\begin{itemize}
  \item One issue is that we cannot easily ``square up'' the linear system to be of size $K \times K$,
    because increasing the degree of the polynomials to $K$ adds $C_K^{(N)} - C_n^{(N)} > K-n$ coefficients
    if $N>1$. So we would need to add the ``right'' number of coefficients.
  \item We could simply try and solve the nonconvex least-squares problem \eqref{eq:PadeLS} for the
    coefficients ... Sven can try this on some examples.
  \item Outline how the linear algebra generalizes to dimension $N$.
\end{itemize}



==> numerics-old.tex <==
\section{Numerical Experiments}\label{SEC:numerics}

\textcolor{blue}{would be good to give here a very brief mention of what aspects will be compared (performance, time, robustness/errors?}
The numerical experiments are conducted on four compute nodes running on Ubuntu 16.04. Each compute node has a 2X Intel Xeon Gold CPU running at 2.10GHz. Additionally, each compute node is equipped with 192GB DDR4 2666 MHz Memory. The code is written in Python v3.7.2 where the optimization functions and constraints are compiled using Numba JIT compiler v0.42.

The experiments are conducted on test problems whose functional forms are summarized in Table~\ref{T:TPs}. The interpolation points $\{x^{(0)},\dots,x^{(K-1)}\}$ are randomly chosen from the \textit{Domain}. 
Each functional value $y^{(k)}$ is obtained by evaluating \textit{f} at $x^{(k)}$.  
The number of interpolation points \textit{K} is always twice the total degrees of freedom of the polynomials in each approximation given by $\alpha(M)$ + $\alpha(N)$ for numerator of degree $M$ and denominator of degree $N$.
We consider both noise-free and noisy data in the experiments. For noisy data, each functional value $y^{(k)}$ is multiplied with a  percentage $\epsilon$ of random value $\phi^{(k)}$ sampled from a standard normal distribution $\mathcal{N}(0,1)$ as follows:
\begin{equation}\label{eq:noise}
y^{(k)} = f(x^{(k)}) [1+\epsilon\phi^{(k)}],\quad\forall k=0,\dots,K-1
\end{equation} 
The approximation $r(x)$ is computed as 
\begin{equation}\label{eq:rofxopts}
r(x) =\left\{
\begin{array}{ll}
\frac{\strut p(x)}{\strut    1} & \text{polynomial approximation}\\
\frac{\strut p(x)}{\strut q(x)} & \text{rational approximation using algorithm~\ref{ALG:MVVandQR}}\\
\frac{\strut p(x)}{\strut q(x)} & \text{rational approximation using algorithm~\ref{A:Polyak}}
\end{array}
\right.    
\end{equation}
where the polynomial approximation is computed by a \textit{NumPy} implementation of finding the linear least-squares solution using singular value decomposition with an algorithm based on divide and conquer within the driver routine \textit{DGELSD}~\cite{laug}.
 
Additionally, we choose another set of interpolation points $\{x^{(K)},\dots,x^{(L-1)}\}$ for testing and compute their functional values $\{f(x^{(K)}),\dots,f(x^{(L-1)})\}$. No noise is added to the testing data. 
The test metric used to compare the quality of the approximation $r(x)$ is
\begin{equation}\label{eq:testError}
\Delta_r = \left|\left|r - f\right|\right|_2 \approx \left[\sum\limits_{k = K}^{L-1} (r(x^{(k)}) - f(x^{(k)}) )^2\right]^{1/2}
\end{equation}
We consider a solution to be better if it has lower $\Delta_r$. 
Finally, in this section, it is assumed that the degrees of numerator and denominator polynomials of the approximations are given. A heuristic algorithm for choosing the ``optimal" degrees of the polynomials is discussed in Section~\ref{SEC:degree}.

%%% ========================================================================== %%%

\subsection{Effect of Constraints on Rational Approximation}\label{sec:numconstrra}
\textcolor{blue}{I would move this section to the algorithm description -- like an illustration of the constraint handling.}
In this section, we examine the effects of constraints on the rational approximation computed using the constrained optimization approach described in Section~\ref{SEC:opti}. 
\cref{fig:imap} shows the surface plots of the denominator polynomial $q_l(x)$ obtained in three iterations  as well as the rational approximation $p_l(x)/q_l(x)$ obtained in the third iteration of Algorithm~\ref{A:Polyak}. 
The black dots indicate  the location of the minimum of $q_l(x)$.
The blue curve represents the intersection of  $q_l(x)$  with the peach colored plane of poles, i.e.,  the blue curve shows the poles in $q_l(x)$. 
In each iteration of Algorithm~\ref{A:Polyak} (line 7), we add the minimum point  as a constraint to \eqref{eq:rationalApproxFD}. Thus, this part of the surface is ``pushed up'' and the poles disappear as illustrated in \cref{fig:imapq2} and \cref{fig:imapq3}. Thus, the final rational approximation  at the end of Algorithm~\ref{A:Polyak} is free of poles.

\begin{figure}[htb!]
	\centering
	\begin{subfigure}[b]{0.49\textwidth}
		\centering
		\includegraphics[width=.8\textwidth]{images/iterationmapq1.png}
		\caption{Surface plot for $q_1(x)$}    
		\label{fig:imapq1}
	\end{subfigure}
	%	\hfill
	\begin{subfigure}[b]{0.49\textwidth}  
		\centering
		\includegraphics[width=.8\textwidth]{images/iterationmapq2.png}
		\caption{Surface plot for $q_2(x)$}    
		\label{fig:imapq2}
	\end{subfigure}
	\vskip\baselineskip
	\begin{subfigure}[b]{0.49\textwidth}
		\centering
		\includegraphics[width=.8\textwidth]{images/iterationmapq3.png}
		\caption{Surface plot for $q_3(x)$}        
		\label{fig:imapq3}
	\end{subfigure}
	%	\hfill
	\begin{subfigure}[b]{0.4\textwidth}  
		\centering
		\includegraphics[width=.8\textwidth]{images/iterationmappq.png}
		\caption{Surface plot for $\frac{p_3(x)}{q_3(x)}$}        
		\label{fig:imappq}
	\end{subfigure}
	\caption{Shown are three iterations of Algorithm~\ref{A:Polyak}. The black dot represents the \textcolor{blue}{global?} minimum of $q_l(x)$; the blue curve represents the poles of $q_l(x)$. In each iteration, we add the minimum point as a constraint to \eqref{eq:rationalApproxFD}. Thus, we keep  removing poles until the final $q_l(x)$ is pole-free. \textcolor{blue}{increase font in figures}}
	\label{fig:imap}
\end{figure}


%%% ========================================================================== %%%
\subsection{Comparing Polynomial and Rational Approximation Quality}

In this section, we compare the approximation quality of the polynomials and the two
rational approximations, namely the approach based on linear algebra described in Section~\ref{SEC:LinAlg}, and that based on constrained optimization described in Section~\ref{SEC:opti}.
We examine the approximation quality for rational, non-rational, and polynomial functions from \cref{T:TPs} with noise-fee and noisy interpolation data.

To compare the quality of the two rational approximations, we examine their testing error as well as the errors with and without poles.
To do this, we first find the set of  points that have a pole-like behavior, which is obtained as
\begin{equation}\label{eq:noofpoles}
W_{r,t} = \left\{j | \frac{|r(x^{(j)})|}{\max\left(1,|f_{max}|\right)} > t, \textcolor{blue}{j = K,\ldots, L-1?}\right\}
 \end{equation}
 where $f_{max}$ is the maximum value of the original function and $t$ is a large threshold. 
 Then, the error due to poles is given as
 \begin{equation}\label{eq:errorfrompoles}
E_{r,t} = \left[\sum\limits_{j \in W_{r,t}} (r(x^{(j)}) - f(x^{(j)}) )^2\right]^{1/2}
\end{equation}
and the error without poles is
\begin{equation}\label{eq:errornotfrompoles}
E'_{r,t} = \left[\Delta_r^2 - E_{r,t}^2\right]^{1/2}
\end{equation}

\cref{tab:poles} describes the results obtained from the comparison of  the quality of the two rational approximations. It can be observed that the approximation based on linear algebra using Algorithm~\ref{ALG:MVVandQR} exhibits pole-like behavior that the approximation based on constrained optimization using Algorithm~\ref{A:Polyak}, does not. As discussed in Section~\ref{sec:numconstrra}, this is due to the iterative removal of poles by Algorithm~\ref{A:Polyak}. 
Moreover, whenever poles are found, the error is quite high, which is due to the definition of \eqref{eq:errorfrompoles}. 
However, the approximation using Algorithm~\ref{ALG:MVVandQR}  is not as good as the approximation using Algorithm~\ref{A:Polyak} since its error without poles is higher.

The approximations using noise-free data are better than for noisy data. This is because the degree of the numerator and denominator polynomials are the same in both the noise-free and the noisy cases. 
Thus, for a high level of noise,  e.g., $\epsilon=10^{-1}$, the approximations underfit the data, causing larger errors. 
Hence, to better fit the noisy data, the approximation requires different degrees of freedom, which is discussed further in Section~\ref{SEC:degree}.
Additionally, in the noisy data case, more pole-like behavior can be observed in the approximation using Algorithm~\ref{ALG:MVVandQR} and this contributes to even larger errors. 

%###################################################
\clearpage

%TODO
%Poles -- 4 tables lhs,mc,sg,sc) -- for sg no M and SD as only 1 exp is run
%for all tables except sg
%FNo. 																eps = 0						eps = 10-1
%																RA					RASIP		RA		RASIP
%														t=100	t=1000 ...
%														M	SD	M	SD	...
%|				W_r,t^(in)|/total
%				|W_r,t^(iout)|/total
%							E_r,t
%							E'_r,t
%							delta_r

 \begin{table}[htb!]
% 	\resizebox{\columnwidth}{!}{%
		\scriptsize
 		\centering
 		\caption{Comparison of the quality of rational approximation \textcolor{red}{Sampling strategy: Uniform random, $\epsilon = 0$}
 			\textcolor{blue}{--explain $\epsilon$, $t$, etc in caption; \textbf{bold} whats important?}} \label{tab:poles}
 		\setlength{\tabcolsep}{5pt}
 		\begin{tabular}{|*{15}{c|}} 
% 			{cc|c|c|c|c|c|c|c|c|c|c|c|c|}
% 			\cline{3-15}
% 			\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
% 			&\multicolumn{6}{|c|}{$\epsilon=0$}
% 			&\multicolumn{6}{|c|}{$\epsilon=10^{-1}$}
% 			\\
 			\cline{4-15}
 			\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
 			&\multicolumn{4}{|c|}{RA w/o Deg. Red.}
 			&\multicolumn{4}{|c|}{RA w/ Deg. Red.}
 			&\multicolumn{4}{|c|}{Pole Free RA}
 			\\
 			\cline{4-15}
			\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
 			&\multicolumn{2}{|c|}{$t=10^2$}
 			&\multicolumn{2}{|c|}{$t=10^3$}
 			&\multicolumn{2}{|c|}{$t=10^2$}
 			&\multicolumn{2}{|c|}{$t=10^3$}
 			&\multicolumn{2}{|c|}{$t=10^2$}
 			&\multicolumn{2}{|c|}{$t=10^3$}
 			\\
 			\cline{1-15}
			\multicolumn{1}{|c|}{FNo.}
			&&\textit{N}&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
			&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
			&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
			\\
			\cline{1-15}\hline\hline
%			MC 0
			
			
			\multirow{2}{*}{\ref{fn:f1}}&$|W_{r,t}^{cner}|/N$&4.0E+05&6.5E-06&5.8E-06&1.0E-06&1.2E-06&6.5E-06&5.8E-06&1.0E-06&1.2E-06&0&0&0&0\\\cline{2-15}
			&$|W_{r,t}^{in}|/N$&1.0E+06&6.0E-07&4.9E-07&0&0&6.0E-07&4.9E-07&0&0&0&0&0&0\\\cline{2-15}
			\hline
			\multirow{2}{*}{\ref{fn:f2}}&$|W_{r,t}^{cner}|/N$&4.0E+05&2.3E-05&3.4E-05&2.0E-06&2.9E-06&2.3E-05&3.4E-05&2.0E-06&2.9E-06&0&0&0&0\\\cline{2-15}
			&$|W_{r,t}^{in}|/N$&1.0E+06&6.0E-07&1.2E-06&0&0&6.0E-07&1.2E-06&0&0&0&0&0&0\\\cline{2-15}
			\hline
			\multirow{2}{*}{\ref{fn:f3}}&$|W_{r,t}^{cner}|/N$&4.0E+05&1.8E-05&3.6E-05&2.0E-06&4.0E-06&1.8E-05&3.6E-05&2.0E-06&4.0E-06&0&0&0&0\\\cline{2-15}
			&$|W_{r,t}^{in}|/N$&1.0E+06&2.4E-06&2.9E-06&4.0E-07&8.0E-07&2.4E-06&2.9E-06&4.0E-07&8.0E-07&0&0&0&0\\\cline{2-15}
			\hline
			\multirow{2}{*}{\ref{fn:f4}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
			&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
			\hline
			\multirow{2}{*}{\ref{fn:f5}}&$|W_{r,t}^{cner}|/N$&4.0E+05&3.0E-06&4.0E-06&0&0&3.0E-06&4.0E-06&0&0&0&0&0&0\\\cline{2-15}
			&$|W_{r,t}^{in}|/N$&1.0E+06&1.8E-06&1.2E-06&0&0&1.8E-06&1.2E-06&0&0&0&0&0&0\\\cline{2-15}
			\hline
			\multirow{2}{*}{\ref{fn:f7}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
			&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
			\hline
			\multirow{2}{*}{\ref{fn:f8}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
			&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
			\hline
			\multirow{2}{*}{\ref{fn:f9}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
			&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
			\hline
			\multirow{2}{*}{\ref{fn:f10}}&$|W_{r,t}^{cner}|/N$&7.9E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
			&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
			\hline
			\multirow{2}{*}{\ref{fn:f12}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
			&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
			\hline
			\multirow{2}{*}{\ref{fn:f13}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
			&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
			\hline
			\multirow{2}{*}{\ref{fn:f14}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
			&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
			\hline
			\multirow{2}{*}{\ref{fn:f15}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
			&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
			\hline
			\multirow{2}{*}{\ref{fn:f16}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
			&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
			\hline
			\multirow{2}{*}{\ref{fn:f17}}&$|W_{r,t}^{cner}|/N$&6.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
			&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
			\hline
			\multirow{2}{*}{\ref{fn:f18}}&$|W_{r,t}^{cner}|/N$&7.9E+05&6.7E-02&3.4E-03&5.7E-03&3.4E-04&6.7E-02&3.4E-03&5.7E-03&3.4E-04&4.2E-02&2.5E-03&4.0E-04&3.1E-04\\\cline{2-15}
			&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
			\hline
			\multirow{2}{*}{\ref{fn:f19}}&$|W_{r,t}^{cner}|/N$&7.9E+05&3.3E-06&6.2E-07&0&0&3.3E-06&6.2E-07&0&0&0&0&0&0\\\cline{2-15}
			&$|W_{r,t}^{in}|/N$&1.0E+06&8.0E-07&7.5E-07&2.0E-07&4.0E-07&8.0E-07&7.5E-07&2.0E-07&4.0E-07&0&0&0&0\\\cline{2-15}
			\hline
			\multirow{2}{*}{\ref{fn:f20}}&$|W_{r,t}^{cner}|/N$&7.9E+05&1.3E-06&1.1E-06&2.5E-07&5.1E-07&1.3E-06&1.1E-06&2.5E-07&5.1E-07&0&0&0&0\\\cline{2-15}
			&$|W_{r,t}^{in}|/N$&1.0E+06&1.6E-06&8.0E-07&0&0&1.6E-06&8.0E-07&0&0&0&0&0&0\\\cline{2-15}
			\hline
			\multirow{2}{*}{\ref{fn:f21}}&$|W_{r,t}^{cner}|/N$&4.0E+05&4.4E-04&1.4E-04&4.8E-05&2.3E-05&4.4E-04&1.4E-04&4.8E-05&2.3E-05&0&0&0&0\\\cline{2-15}
			&$|W_{r,t}^{in}|/N$&1.0E+06&2.2E-04&8.6E-05&2.3E-05&8.6E-06&2.2E-04&8.6E-05&2.3E-05&8.6E-06&0&0&0&0\\\cline{2-15}
			\hline
			\multirow{2}{*}{\ref{fn:f22}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
			&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
			\hline
			
 		\end{tabular}
% 	}
 \end{table}

 \begin{table}[htb!]
	% 	\resizebox{\columnwidth}{!}{%
	\scriptsize
	\centering
	\caption{\textcolor{red}{Sampling strategy: Uniform random, $\epsilon = 10^{-6}$}
		\textcolor{blue}{--explain $\epsilon$, $t$, etc in caption; \textbf{bold} whats important?}} \label{tab:poles11}
	\setlength{\tabcolsep}{5pt}
	\begin{tabular}{|*{15}{c|}} 
		% 			{cc|c|c|c|c|c|c|c|c|c|c|c|c|}
		% 			\cline{3-15}
		% 			\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		% 			&\multicolumn{6}{|c|}{$\epsilon=0$}
		% 			&\multicolumn{6}{|c|}{$\epsilon=10^{-1}$}
		% 			\\
		\cline{4-15}
		\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\multicolumn{4}{|c|}{RA w/o Deg. Red.}
		&\multicolumn{4}{|c|}{RA w/ Deg. Red.}
		&\multicolumn{4}{|c|}{Pole Free RA}
		\\
		\cline{4-15}
		\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		\\
		\cline{1-15}
		\multicolumn{1}{|c|}{FNo.}
		&&\textit{N}&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		\\
		\cline{1-15}\hline\hline
%		MC 10-6
		
		
		\multirow{2}{*}{\ref{fn:f1}}&$|W_{r,t}^{cner}|/N$&4.0E+05&8.5E-06&3.7E-06&5.0E-07&1.0E-06&8.5E-06&3.7E-06&5.0E-07&1.0E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&4.0E-07&8.0E-07&4.0E-07&8.0E-07&4.0E-07&8.0E-0\left( 7&4.0E-07&8.0E-07&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f2}}&$|W_{r,t}^{cner}|/N$&4.0E+05&1.6E-05&3.0E-05&1.5E-06&3.0E-06&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.4E-06&1.9E-06&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f3}}&$|W_{r,t}^{cner}|/N$&4.0E+05&2.0E-06&4.0E-06&0&0&5.0E-05&1.0E-04&8.5E-06&1.7E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&2.0E-06&2.5E-06&0&0&2.9E-05&5.5E-05&2.8E-06&5.6E-06&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f4}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f5}}&$|W_{r,t}^{cner}|/N$&4.0E+05&2.0E-06&4.0E-06&0&0&6.4E-05&9.4E-05&2.3E-05&3.9E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&8.0E-07&4.0E-07&0&0&4.2E-05&3.1E-05&7.2E-06&5.6E-06&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f7}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f8}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f9}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&1.2E-05&2.4E-05&1.0E-06&2.0E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&4.6E-06&9.2E-06&6.0E-07&1.2E-06&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f10}}&$|W_{r,t}^{cner}|/N$&7.9E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f12}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f13}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&8.5E-05&1.7E-04&3.5E-06&7.0E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&1.5E-05&2.9E-05&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f14}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&2.1E-05&4.3E-05&1.5E-06&3.0E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&9.6E-06&1.9E-05&1.0E-06&2.0E-06&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f15}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&6.4E-05&1.3E-04&6.5E-06&1.3E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&2.2E-05&4.4E-05&3.2E-06&6.4E-06&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f16}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&1.9E-04&1.3E-04&2.3E-05&1.6E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&3.0E-05&1.3E-05&3.4E-06&3.0E-06&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f17}}&$|W_{r,t}^{cner}|/N$&6.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f18}}&$|W_{r,t}^{cner}|/N$&7.9E+05&6.7E-02&3.4E-03&5.7E-03&3.4E-04&6.7E-02&3.4E-03&5.7E-03&3.4E-04&4.2E-02&2.3E-03&1.4E-04&1.1E-04\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f19}}&$|W_{r,t}^{cner}|/N$&7.9E+05&3.3E-06&1.3E-06&5.1E-07&6.2E-07&3.3E-06&1.3E-06&5.1E-07&6.2E-07&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.2E-06&7.5E-07&0&0&1.2E-06&7.5E-07&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f20}}&$|W_{r,t}^{cner}|/N$&7.9E+05&1.5E-06&1.2E-06&0&0&2.5E-07&5.1E-07&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.2E-06&4.0E-07&2.0E-07&4.0E-07&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f21}}&$|W_{r,t}^{cner}|/N$&4.0E+05&4.4E-04&1.4E-04&4.8E-05&2.3E-05&5.6E-05&4.3E-05&6.5E-06&7.2E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&2.2E-04&8.6E-05&2.3E-05&8.6E-06&6.8E-05&3.6E-05&5.0E-06&2.4E-06&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f22}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		
	\end{tabular}
	% 	}
\end{table}

 \begin{table}[htb!]
	% 	\resizebox{\columnwidth}{!}{%
	\scriptsize
	\centering
	\caption{\textcolor{red}{Sampling strategy: Uniform random, $\epsilon = 10^{-2}$}
		\textcolor{blue}{--explain $\epsilon$, $t$, etc in caption; \textbf{bold} whats important?}} \label{tab:poles12}
	\setlength{\tabcolsep}{5pt}
	\begin{tabular}{|*{15}{c|}} 
		% 			{cc|c|c|c|c|c|c|c|c|c|c|c|c|}
		% 			\cline{3-15}
		% 			\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		% 			&\multicolumn{6}{|c|}{$\epsilon=0$}
		% 			&\multicolumn{6}{|c|}{$\epsilon=10^{-1}$}
		% 			\\
		\cline{4-15}
		\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\multicolumn{4}{|c|}{RA w/o Deg. Red.}
		&\multicolumn{4}{|c|}{RA w/ Deg. Red.}
		&\multicolumn{4}{|c|}{Pole Free RA}
		\\
		\cline{4-15}
		\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		\\
		\cline{1-15}
		\multicolumn{1}{|c|}{FNo.}
		&&\textit{N}&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		\\
		\cline{1-15}\hline\hline
		%		MC 10-2
		
		\multirow{2}{*}{\ref{fn:f1}}&$|W_{r,t}^{cner}|/N$&4.0E+05&6.1E-05&6.3E-05&6.5E-06&5.4E-06&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.4E-05&1.3E-05&2.2E-06&2.5E-06&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f2}}&$|W_{r,t}^{cner}|/N$&4.0E+05&1.4E-04&1.2E-04&9.0E-06&2.5E-06&1.2E-03&4.6E-04&1.1E-04&2.0E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&3.3E-05&1.5E-05&2.2E-06&1.8E-06&1.0E-03&1.6E-04&9.7E-05&1.5E-05&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f3}}&$|W_{r,t}^{cner}|/N$&4.0E+05&4.3E-04&3.4E-04&1.6E-05&2.1E-05&2.1E-03&2.1E-03&2.3E-04&2.5E-04&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&2.4E-04&1.1E-04&2.3E-05&1.3E-05&2.7E-03&7.3E-04&2.7E-04&7.8E-05&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f4}}&$|W_{r,t}^{cner}|/N$&4.0E+05&1.9E-05&8.2E-06&3.0E-06&2.4E-06&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&3.9E-05&1.0E-05&4.0E-06&2.4E-06&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f5}}&$|W_{r,t}^{cner}|/N$&4.0E+05&5.1E-05&7.9E-05&5.0E-06&8.8E-06&3.2E-04&2.4E-04&2.9E-05&2.2E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.9E-05&6.8E-06&2.0E-06&1.4E-06&4.9E-04&1.5E-04&5.3E-05&1.5E-05&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f7}}&$|W_{r,t}^{cner}|/N$&4.0E+05&1.4E-04&1.5E-04&8.5E-06&8.5E-06&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&3.9E-05&3.0E-05&5.2E-06&4.4E-06&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f8}}&$|W_{r,t}^{cner}|/N$&4.0E+05&1.0E-06&1.2E-06&0&0&5.9E-04&5.9E-04&5.8E-05&5.8E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.0E-06&1.3E-06&0&0&2.6E-05&2.1E-05&1.4E-06&1.4E-06&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f9}}&$|W_{r,t}^{cner}|/N$&4.0E+05&1.8E-05&2.6E-05&1.5E-06&3.0E-06&7.0E-06&6.6E-06&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&4.0E-07&4.9E-07&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f10}}&$|W_{r,t}^{cner}|/N$&7.9E+05&7.6E-06&3.6E-06&7.6E-07&6.2E-07&9.2E-05&3.8E-05&7.9E-06&6.4E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&4.2E-06&9.8E-07&6.0E-07&4.9E-07&1.2E-05&6.4E-06&1.8E-06&1.5E-06&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f12}}&$|W_{r,t}^{cner}|/N$&4.0E+05&4.5E-05&7.5E-05&4.5E-06&6.8E-06&3.5E-04&2.1E-04&4.3E-05&2.7E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.6E-05&6.4E-06&2.0E-06&8.9E-07&5.2E-04&1.9E-04&5.2E-05&2.4E-05&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f13}}&$|W_{r,t}^{cner}|/N$&4.0E+05&4.5E-06&1.9E-06&1.0E-06&2.0E-06&8.1E-05&5.2E-05&7.0E-06&5.1E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&4.4E-06&1.0E-06&6.0E-07&8.0E-07&5.2E-05&3.2E-05&4.6E-06&3.7E-06&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f14}}&$|W_{r,t}^{cner}|/N$&4.0E+05&1.7E-05&1.7E-05&1.5E-06&2.0E-06&2.3E-04&1.5E-04&2.3E-05&1.5E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&2.2E-06&1.6E-06&0&0&5.8E-06&3.9E-06&8.0E-07&4.0E-07&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f15}}&$|W_{r,t}^{cner}|/N$&4.0E+05&5.6E-05&3.9E-05&5.0E-06&4.5E-06&3.2E-05&5.4E-05&3.5E-06&7.0E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&8.4E-06&6.9E-06&8.0E-07&4.0E-07&1.4E-05&1.1E-05&2.0E-06&1.7E-06&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f16}}&$|W_{r,t}^{cner}|/N$&4.0E+05&1.1E-05&8.6E-06&1.0E-06&1.2E-06&3.0E-04&1.2E-04&3.4E-05&1.3E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.2E-06&1.2E-06&2.0E-07&4.0E-07&5.0E-06&3.3E-06&8.0E-07&9.8E-07&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f17}}&$|W_{r,t}^{cner}|/N$&6.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f18}}&$|W_{r,t}^{cner}|/N$&7.9E+05&6.9E-02&5.8E-03&5.5E-03&1.1E-03&1.1E-03&7.4E-04&1.1E-04&7.5E-05&3.9E-02&2.1E-03&1.4E-04&1.8E-04\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f19}}&$|W_{r,t}^{cner}|/N$&7.9E+05&3.8E-05&9.7E-06&2.3E-06&2.0E-06&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.9E-05&3.2E-06&1.6E-06&1.7E-06&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f20}}&$|W_{r,t}^{cner}|/N$&7.9E+05&2.0E-06&1.0E-06&5.1E-07&1.0E-06&1.3E-06&2.5E-06&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.8E-06&1.9E-06&2.0E-07&4.0E-07&2.0E-07&4.0E-07&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f21}}&$|W_{r,t}^{cner}|/N$&4.0E+05&3.2E-04&1.6E-04&4.8E-05&2.8E-05&1.4E-05&1.8E-05&1.0E-06&1.2E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&2.2E-04&8.1E-05&2.3E-05&7.4E-06&6.8E-06&5.2E-06&1.2E-06&7.5E-07&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f22}}&$|W_{r,t}^{cner}|/N$&4.0E+05&1.4E-05&1.7E-05&2.0E-06&1.9E-06&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.4E-05&1.0E-05&8.0E-07&4.0E-07&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		
		
	\end{tabular}
	% 	}
\end{table}

 \begin{table}[htb!]
	% 	\resizebox{\columnwidth}{!}{%
	\scriptsize
	\centering
	\caption{\textcolor{red}{Sampling strategy: Latin Hypercube Sampling, $\epsilon = 0$}
		\textcolor{blue}{--explain $\epsilon$, $t$, etc in caption; \textbf{bold} whats important?}} \label{tab:poles20}
	\setlength{\tabcolsep}{5pt}
	\begin{tabular}{|*{15}{c|}} 
		% 			{cc|c|c|c|c|c|c|c|c|c|c|c|c|}
		% 			\cline{3-15}
		% 			\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		% 			&\multicolumn{6}{|c|}{$\epsilon=0$}
		% 			&\multicolumn{6}{|c|}{$\epsilon=10^{-1}$}
		% 			\\
		\cline{4-15}
		\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\multicolumn{4}{|c|}{RA w/o Deg. Red.}
		&\multicolumn{4}{|c|}{RA w/ Deg. Red.}
		&\multicolumn{4}{|c|}{Pole Free RA}
		\\
		\cline{4-15}
		\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		\\
		\cline{1-15}
		\multicolumn{1}{|c|}{FNo.}
		&&\textit{N}&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		\\
		\cline{1-15}\hline\hline
		%	LHS 0
		
		\multirow{2}{*}{\ref{fn:f1}}&$|W_{r,t}^{cner}|/N$&4.0E+05&1.5E-06&2.0E-06&0&0&1.5E-06&2.0E-06&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f2}}&$|W_{r,t}^{cner}|/N$&4.0E+05&5.5E-06&8.6E-06&5.0E-07&1.0E-06&5.5E-06&8.6E-06&5.0E-07&1.0E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f3}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f4}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f5}}&$|W_{r,t}^{cner}|/N$&4.0E+05&1.0E-06&1.2E-06&5.0E-07&1.0E-06&1.0E-06&1.2E-06&5.0E-07&1.0E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.0E-06&8.9E-07&0&0&1.0E-06&8.9E-07&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f7}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f8}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f9}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f10}}&$|W_{r,t}^{cner}|/N$&7.9E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f12}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f13}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f14}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f15}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f16}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f17}}&$|W_{r,t}^{cner}|/N$&6.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f18}}&$|W_{r,t}^{cner}|/N$&7.9E+05&5.6E-02&6.4E-03&4.6E-03&9.1E-04&5.6E-02&6.4E-03&4.6E-03&9.1E-04&2.0E-02&4.4E-03&9.2E-06&1.8E-05\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f19}}&$|W_{r,t}^{cner}|/N$&7.9E+05&2.8E-06&2.5E-06&2.5E-07&5.1E-07&2.8E-06&2.5E-06&2.5E-07&5.1E-07&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.4E-06&1.0E-06&0&0&1.4E-06&1.0E-06&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f20}}&$|W_{r,t}^{cner}|/N$&7.9E+05&3.1E-06&6.2E-07&2.5E-07&5.1E-07&3.1E-06&6.2E-07&2.5E-07&5.1E-07&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&2.0E-06&1.3E-06&2.0E-07&4.0E-07&2.0E-06&1.3E-06&2.0E-07&4.0E-07&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f21}}&$|W_{r,t}^{cner}|/N$&4.0E+05&4.6E-04&2.1E-04&6.2E-05&4.5E-05&4.6E-04&2.1E-04&6.2E-05&4.5E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.9E-04&6.1E-05&2.0E-05&9.0E-06&1.9E-04&6.1E-05&2.0E-05&9.0E-06&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f22}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		
		
	\end{tabular}
	% 	}
\end{table}

\begin{table}[htb!]
	% 	\resizebox{\columnwidth}{!}{%
	\scriptsize
	\centering
	\caption{\textcolor{red}{Sampling strategy: Latin Hypercube Sampling, $\epsilon = 10^{-6}$}
		\textcolor{blue}{--explain $\epsilon$, $t$, etc in caption; \textbf{bold} whats important?}} \label{tab:poles21}
	\setlength{\tabcolsep}{5pt}
	\begin{tabular}{|*{15}{c|}} 
		% 			{cc|c|c|c|c|c|c|c|c|c|c|c|c|}
		% 			\cline{3-15}
		% 			\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		% 			&\multicolumn{6}{|c|}{$\epsilon=0$}
		% 			&\multicolumn{6}{|c|}{$\epsilon=10^{-1}$}
		% 			\\
		\cline{4-15}
		\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\multicolumn{4}{|c|}{RA w/o Deg. Red.}
		&\multicolumn{4}{|c|}{RA w/ Deg. Red.}
		&\multicolumn{4}{|c|}{Pole Free RA}
		\\
		\cline{4-15}
		\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		\\
		\cline{1-15}
		\multicolumn{1}{|c|}{FNo.}
		&&\textit{N}&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		\\
		\cline{1-15}\hline\hline
		%		LHS 10-6
		
		\multirow{2}{*}{\ref{fn:f1}}&$|W_{r,t}^{cner}|/N$&4.0E+05&1.5E-06&2.0E-06&0&0&1.5E-06&2.0E-06&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f2}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&3.0E-06&3.7E-06&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&6.0E-07&8.0E-07&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f3}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&5.7E-05&8.6E-05&5.0E-06&7.7E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&8.4E-05&1.1E-04&9.4E-06&1.2E-05&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f4}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f5}}&$|W_{r,t}^{cner}|/N$&4.0E+05&5.0E-07&1.0E-06&0&0&3.6E-04&3.4E-04&3.1E-05&2.4E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.2E-06&9.8E-07&2.0E-07&4.0E-07&2.2E-04&1.6E-04&2.4E-05&2.0E-05&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f7}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f8}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f9}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&2.5E-06&5.0E-06&5.0E-07&1.0E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&2.2E-06&4.4E-06&4.0E-07&8.0E-07&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f10}}&$|W_{r,t}^{cner}|/N$&7.9E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f12}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f13}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&1.4E-04&2.1E-04&3.9E-05&7.0E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&1.2E-04&1.0E-04&1.2E-05&1.1E-05&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f14}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&8.7E-05&1.1E-04&8.5E-06&1.1E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&2.8E-05&4.5E-05&2.0E-06&3.5E-06&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f15}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&5.5E-05&1.1E-04&5.5E-06&1.1E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&6.1E-05&1.2E-04&5.2E-06&1.0E-05&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f16}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&1.8E-04&1.4E-04&2.0E-05&1.7E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&6.1E-05&6.7E-05&5.8E-06&6.8E-06&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f17}}&$|W_{r,t}^{cner}|/N$&6.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f18}}&$|W_{r,t}^{cner}|/N$&7.9E+05&5.6E-02&6.4E-03&4.6E-03&9.1E-04&5.8E-02&9.1E-03&4.9E-03&1.2E-03&2.1E-02&4.0E-03&1.4E-05&2.7E-05\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f19}}&$|W_{r,t}^{cner}|/N$&7.9E+05&3.3E-06&2.7E-06&2.5E-07&5.1E-07&3.3E-06&2.7E-06&2.5E-07&5.1E-07&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&8.0E-07&7.5E-07&0&0&8.0E-07&7.5E-07&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f20}}&$|W_{r,t}^{cner}|/N$&7.9E+05&2.5E-06&1.4E-06&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.8E-06&1.3E-06&2.0E-07&4.0E-07&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f21}}&$|W_{r,t}^{cner}|/N$&4.0E+05&4.6E-04&2.1E-04&6.1E-05&4.4E-05&3.5E-05&3.4E-05&2.5E-06&2.2E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.9E-04&6.0E-05&2.0E-05&9.4E-06&5.9E-05&3.7E-05&7.2E-06&3.4E-06&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f22}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		
		
	\end{tabular}
	% 	}
\end{table}

\begin{table}[htb!]
	% 	\resizebox{\columnwidth}{!}{%
	\scriptsize
	\centering
	\caption{\textcolor{red}{Sampling strategy: Latin Hypercube Sampling, $\epsilon = 10^{-2}$}
		\textcolor{blue}{--explain $\epsilon$, $t$, etc in caption; \textbf{bold} whats important?}} \label{tab:poles22}
	\setlength{\tabcolsep}{5pt}
	\begin{tabular}{|*{15}{c|}} 
		% 			{cc|c|c|c|c|c|c|c|c|c|c|c|c|}
		% 			\cline{3-15}
		% 			\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		% 			&\multicolumn{6}{|c|}{$\epsilon=0$}
		% 			&\multicolumn{6}{|c|}{$\epsilon=10^{-1}$}
		% 			\\
		\cline{4-15}
		\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\multicolumn{4}{|c|}{RA w/o Deg. Red.}
		&\multicolumn{4}{|c|}{RA w/ Deg. Red.}
		&\multicolumn{4}{|c|}{Pole Free RA}
		\\
		\cline{4-15}
		\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		\\
		\cline{1-15}\hline\hline
		%		LHS 10-2
		
		\multirow{2}{*}{\ref{fn:f1}}&$|W_{r,t}^{cner}|/N$&4.0E+05&7.7E-04&3.7E-04&9.2E-05&7.3E-05&4.6E-04&6.3E-05&4.0E-05&5.1E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&6.4E-05&8.7E-05&4.8E-06&6.7E-06&7.5E-05&1.0E-05&7.0E-06&3.8E-06&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f2}}&$|W_{r,t}^{cner}|/N$&4.0E+05&3.2E-05&1.2E-05&2.5E-06&1.6E-06&8.5E-04&4.5E-04&4.8E-05&3.1E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&2.2E-05&9.8E-06&3.2E-06&2.9E-06&7.0E-04&1.6E-04&7.0E-05&1.6E-05&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f3}}&$|W_{r,t}^{cner}|/N$&4.0E+05&1.5E-04&1.7E-04&1.6E-05&1.7E-05&3.7E-03&3.1E-03&2.9E-04&2.7E-04&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.0E-04&7.3E-05&9.2E-06&7.2E-06&2.8E-03&2.7E-04&2.9E-04&3.3E-05&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f4}}&$|W_{r,t}^{cner}|/N$&4.0E+05&1.8E-05&1.2E-05&1.5E-06&2.0E-06&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&3.0E-05&8.4E-06&3.6E-06&1.0E-06&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f5}}&$|W_{r,t}^{cner}|/N$&4.0E+05&1.0E-05&9.7E-06&5.0E-07&1.0E-06&4.1E-04&3.6E-04&3.5E-05&2.7E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&7.0E-06&2.8E-06&8.0E-07&7.5E-07&3.8E-04&1.4E-04&4.0E-05&1.2E-05&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f7}}&$|W_{r,t}^{cner}|/N$&4.0E+05&1.3E-04&1.5E-04&3.0E-06&2.9E-06&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&4.1E-05&2.9E-05&4.6E-06&3.8E-06&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f8}}&$|W_{r,t}^{cner}|/N$&4.0E+05&7.8E-05&1.1E-04&6.5E-06&1.2E-05&6.9E-05&1.0E-04&3.0E-06&2.9E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&9.2E-06&1.0E-05&1.8E-06&2.2E-06&7.9E-05&3.9E-05&4.4E-06&3.1E-06&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f9}}&$|W_{r,t}^{cner}|/N$&4.0E+05&9.9E-05&7.2E-05&1.1E-05&9.3E-06&3.1E-05&5.4E-06&4.0E-06&1.2E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&6.6E-06&4.5E-06&1.6E-06&1.2E-06&6.8E-06&1.3E-06&1.4E-06&4.9E-07&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f10}}&$|W_{r,t}^{cner}|/N$&7.9E+05&2.0E-05&1.3E-05&1.3E-06&1.4E-06&1.6E-04&1.5E-05&1.6E-05&2.6E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&9.2E-06&9.8E-07&1.0E-06&1.1E-06&3.1E-05&7.5E-06&2.0E-06&1.3E-06&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f12}}&$|W_{r,t}^{cner}|/N$&4.0E+05&1.3E-05&1.5E-05&2.5E-06&2.7E-06&2.6E-04&2.8E-04&3.4E-05&4.2E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&9.6E-06&6.1E-06&1.8E-06&1.3E-06&6.9E-04&3.9E-04&7.2E-05&4.0E-05&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f13}}&$|W_{r,t}^{cner}|/N$&4.0E+05&7.5E-06&8.8E-06&5.0E-07&1.0E-06&2.4E-04&1.7E-04&4.7E-05&6.1E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&2.4E-06&1.6E-06&4.0E-07&4.9E-07&1.8E-04&1.4E-04&1.6E-05&1.2E-05&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f14}}&$|W_{r,t}^{cner}|/N$&4.0E+05&8.3E-05&9.8E-05&9.0E-06&1.3E-05&3.7E-04&2.3E-05&3.6E-05&3.7E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&2.8E-06&2.7E-06&6.0E-07&1.2E-06&8.1E-05&4.1E-06&9.4E-06&2.1E-06&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f15}}&$|W_{r,t}^{cner}|/N$&4.0E+05&1.0E-04&9.5E-05&1.0E-05&9.6E-06&1.3E-04&1.7E-04&1.4E-05&2.0E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.0E-05&5.8E-06&1.0E-06&1.1E-06&3.3E-05&2.5E-05&3.0E-06&2.2E-06&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f16}}&$|W_{r,t}^{cner}|/N$&4.0E+05&4.3E-05&6.9E-05&4.5E-06&9.0E-06&5.9E-04&4.0E-04&6.0E-05&3.1E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&3.0E-06&4.1E-06&0&0&9.3E-05&3.4E-05&9.2E-06&2.2E-06&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f17}}&$|W_{r,t}^{cner}|/N$&6.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f18}}&$|W_{r,t}^{cner}|/N$&7.9E+05&5.3E-02&5.5E-03&4.5E-03&1.1E-03&1.7E-03&5.7E-04&1.7E-04&5.7E-05&1.8E-02&3.9E-03&2.7E-05&5.3E-05\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f19}}&$|W_{r,t}^{cner}|/N$&7.9E+05&3.6E-05&3.1E-06&3.6E-06&2.0E-06&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.3E-05&4.3E-06&1.0E-06&6.3E-07&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f20}}&$|W_{r,t}^{cner}|/N$&7.9E+05&1.8E-06&1.9E-06&5.1E-07&1.0E-06&5.1E-07&1.0E-06&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.8E-06&7.5E-07&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f21}}&$|W_{r,t}^{cner}|/N$&4.0E+05&5.8E-04&2.4E-04&6.3E-05&4.6E-05&3.9E-05&1.4E-05&4.5E-06&3.3E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&2.0E-04&8.6E-05&2.2E-05&1.4E-05&1.4E-05&4.9E-06&1.6E-06&1.4E-06&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f22}}&$|W_{r,t}^{cner}|/N$&4.0E+05&1.5E-05&1.7E-05&1.5E-06&2.0E-06&1.3E-03&8.7E-05&1.0E-04&6.1E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.0E-05&5.0E-06&6.0E-07&4.9E-07&1.2E-04&5.4E-05&1.4E-05&6.5E-06&0&0&0&0\\\cline{2-15}
		\hline
		
		
	\end{tabular}
	% 	}
\end{table}

 \begin{table}[htb!]
	% 	\resizebox{\columnwidth}{!}{%
	\scriptsize
	\centering
	\caption{\textcolor{red}{Sampling strategy: Sobol Sequence, $\epsilon = 0$}
		\textcolor{blue}{--explain $\epsilon$, $t$, etc in caption; \textbf{bold} whats important?}} \label{tab:poles30}
	\setlength{\tabcolsep}{5pt}
	\begin{tabular}{|*{15}{c|}} 
		% 			{cc|c|c|c|c|c|c|c|c|c|c|c|c|}
		% 			\cline{3-15}
		% 			\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		% 			&\multicolumn{6}{|c|}{$\epsilon=0$}
		% 			&\multicolumn{6}{|c|}{$\epsilon=10^{-1}$}
		% 			\\
		\cline{4-15}
		\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\multicolumn{4}{|c|}{RA w/o Deg. Red.}
		&\multicolumn{4}{|c|}{RA w/ Deg. Red.}
		&\multicolumn{4}{|c|}{Pole Free RA}
		\\
		\cline{4-15}
		\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		\\
		\cline{1-15}
		\multicolumn{1}{|c|}{FNo.}
		&&\textit{N}&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		\\
		\cline{1-15}\hline\hline
		%		SO 0
		
		\multirow{2}{*}{\ref{fn:f1}}&$|W_{r,t}^{cner}|/N$&4.0E+05&2.0E-06&2.4E-06&0&0&2.0E-06&2.4E-06&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&8.0E-07&4.0E-07&2.0E-07&4.0E-07&8.0E-07&4.0E-07&2.0E-07&4.0E-07&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f2}}&$|W_{r,t}^{cner}|/N$&4.0E+05&3.5E-06&5.8E-06&0&0&3.5E-06&5.8E-06&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f3}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f4}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f5}}&$|W_{r,t}^{cner}|/N$&4.0E+05&5.0E-07&1.0E-06&0&0&5.0E-07&1.0E-06&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&4.0E-07&4.9E-07&0&0&4.0E-07&4.9E-07&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f7}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f8}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f9}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f10}}&$|W_{r,t}^{cner}|/N$&7.9E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f12}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f13}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f14}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f15}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f16}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f17}}&$|W_{r,t}^{cner}|/N$&6.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f18}}&$|W_{r,t}^{cner}|/N$&7.9E+05&5.3E-02&7.3E-03&4.4E-03&1.0E-03&5.3E-02&7.3E-03&4.4E-03&1.0E-03&2.2E-02&4.0E-03&2.5E-05&3.6E-05\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f19}}&$|W_{r,t}^{cner}|/N$&7.9E+05&3.8E-06&1.4E-06&7.6E-07&6.2E-07&3.8E-06&1.4E-06&7.6E-07&6.2E-07&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&6.0E-07&8.0E-07&0&0&6.0E-07&8.0E-07&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f20}}&$|W_{r,t}^{cner}|/N$&7.9E+05&2.3E-06&1.5E-06&0&0&2.3E-06&1.5E-06&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&2.4E-06&1.9E-06&8.0E-07&9.8E-07&2.4E-06&1.9E-06&8.0E-07&9.8E-07&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f21}}&$|W_{r,t}^{cner}|/N$&4.0E+05&2.0E-04&1.4E-04&1.7E-05&1.6E-05&2.0E-04&1.4E-04&1.7E-05&1.6E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.9E-04&8.8E-05&1.7E-05&1.1E-05&1.9E-04&8.8E-05&1.7E-05&1.1E-05&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f22}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		
		
		
	\end{tabular}
	% 	}
\end{table}

\begin{table}[htb!]
	% 	\resizebox{\columnwidth}{!}{%
	\scriptsize
	\centering
	\caption{\textcolor{red}{Sampling strategy: Sobol Sequence, $\epsilon = 10^{-6}$}
		\textcolor{blue}{--explain $\epsilon$, $t$, etc in caption; \textbf{bold} whats important?}} \label{tab:poles31}
	\setlength{\tabcolsep}{5pt}
	\begin{tabular}{|*{15}{c|}} 
		% 			{cc|c|c|c|c|c|c|c|c|c|c|c|c|}
		% 			\cline{3-15}
		% 			\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		% 			&\multicolumn{6}{|c|}{$\epsilon=0$}
		% 			&\multicolumn{6}{|c|}{$\epsilon=10^{-1}$}
		% 			\\
		\cline{4-15}
		\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\multicolumn{4}{|c|}{RA w/o Deg. Red.}
		&\multicolumn{4}{|c|}{RA w/ Deg. Red.}
		&\multicolumn{4}{|c|}{Pole Free RA}
		\\
		\cline{4-15}
		\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		\\
		\cline{1-15}
		\multicolumn{1}{|c|}{FNo.}
		&&\textit{N}&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		\\
		\cline{1-15}\hline\hline
		%		SO 10-6
		
		\multirow{2}{*}{\ref{fn:f1}}&$|W_{r,t}^{cner}|/N$&4.0E+05&4.5E-06&2.4E-06&5.0E-07&1.0E-06&4.5E-06&2.4E-06&5.0E-07&1.0E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f2}}&$|W_{r,t}^{cner}|/N$&4.0E+05&5.0E-07&1.0E-06&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&2.0E-07&4.0E-07&0&0&2.0E-07&4.0E-07&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f3}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&5.5E-06&7.1E-06&5.0E-07&1.0E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&1.1E-04&1.6E-04&1.1E-05&1.7E-05&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f4}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f5}}&$|W_{r,t}^{cner}|/N$&4.0E+05&2.5E-06&3.2E-06&5.0E-07&1.0E-06&2.1E-04&2.3E-04&1.9E-05&1.9E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.0E-06&1.1E-06&4.0E-07&4.9E-07&1.4E-04&1.5E-04&1.3E-05&1.2E-05&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f7}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&2.0E-07&4.0E-07&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f8}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f9}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f10}}&$|W_{r,t}^{cner}|/N$&7.9E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f12}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f13}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&1.1E-04&1.6E-04&6.5E-06&8.5E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&1.1E-04&1.1E-04&1.1E-05&1.2E-05&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f14}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&1.2E-05&2.0E-05&1.0E-06&2.0E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&5.0E-06&6.2E-06&2.0E-07&4.0E-07&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f15}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&3.2E-05&6.4E-05&2.0E-06&4.0E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&2.7E-05&5.4E-05&3.4E-06&6.8E-06&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f16}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&2.1E-05&2.3E-05&2.0E-06&1.9E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&1.4E-05&8.4E-06&1.2E-06&1.9E-06&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f17}}&$|W_{r,t}^{cner}|/N$&6.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f18}}&$|W_{r,t}^{cner}|/N$&7.9E+05&5.3E-02&7.3E-03&4.4E-03&1.0E-03&5.3E-02&7.3E-03&4.4E-03&1.0E-03&2.2E-02&2.8E-03&2.0E-04&3.2E-04\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f19}}&$|W_{r,t}^{cner}|/N$&7.9E+05&1.8E-06&1.5E-06&0&0&1.8E-06&1.5E-06&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&8.0E-07&1.2E-06&0&0&8.0E-07&1.2E-06&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f20}}&$|W_{r,t}^{cner}|/N$&7.9E+05&2.3E-06&1.5E-06&2.5E-07&5.1E-07&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.8E-06&1.2E-06&4.0E-07&4.9E-07&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f21}}&$|W_{r,t}^{cner}|/N$&4.0E+05&2.0E-04&1.4E-04&1.6E-05&1.4E-05&3.1E-05&2.3E-05&3.0E-06&3.7E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.9E-04&8.8E-05&1.7E-05&1.1E-05&5.9E-05&2.2E-05&4.8E-06&2.4E-06&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f22}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		
		
	\end{tabular}
	% 	}
\end{table}

\begin{table}[htb!]
	% 	\resizebox{\columnwidth}{!}{%
	\scriptsize
	\centering
	\caption{\textcolor{red}{Sampling strategy: Sobol Sequence, $\epsilon = 10^{-2}$}
		\textcolor{blue}{--explain $\epsilon$, $t$, etc in caption; \textbf{bold} whats important?}} \label{tab:poles32}
	\setlength{\tabcolsep}{5pt}
	\begin{tabular}{|*{15}{c|}} 
		% 			{cc|c|c|c|c|c|c|c|c|c|c|c|c|}
		% 			\cline{3-15}
		% 			\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		% 			&\multicolumn{6}{|c|}{$\epsilon=0$}
		% 			&\multicolumn{6}{|c|}{$\epsilon=10^{-1}$}
		% 			\\
		\cline{4-15}
		\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\multicolumn{4}{|c|}{RA w/o Deg. Red.}
		&\multicolumn{4}{|c|}{RA w/ Deg. Red.}
		&\multicolumn{4}{|c|}{Pole Free RA}
		\\
		\cline{4-15}
		\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		\\
		\cline{1-15}
		\multicolumn{1}{|c|}{FNo.}
		&&\textit{N}&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		\\
		\cline{1-15}\hline\hline
		%		SO 10-2
		
		\multirow{2}{*}{\ref{fn:f1}}&$|W_{r,t}^{cner}|/N$&4.0E+05&3.6E-04&1.7E-04&4.7E-05&2.3E-05&2.9E-04&1.4E-04&3.0E-05&2.2E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&3.1E-05&1.6E-05&2.4E-06&2.1E-06&5.7E-05&2.4E-05&6.4E-06&1.6E-06&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f2}}&$|W_{r,t}^{cner}|/N$&4.0E+05&7.4E-05&8.9E-05&1.1E-05&1.6E-05&7.9E-04&4.7E-04&5.9E-05&4.1E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.9E-05&4.6E-06&6.0E-07&4.9E-07&1.1E-03&7.5E-04&1.1E-04&7.6E-05&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f3}}&$|W_{r,t}^{cner}|/N$&4.0E+05&1.8E-04&1.9E-04&3.3E-05&3.8E-05&6.7E-04&4.4E-04&5.5E-05&6.0E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&5.7E-05&1.5E-05&4.6E-06&1.2E-06&1.9E-03&1.2E-03&1.8E-04&1.1E-04&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f4}}&$|W_{r,t}^{cner}|/N$&4.0E+05&1.9E-05&1.7E-05&2.5E-06&3.2E-06&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&2.7E-05&1.2E-05&3.0E-06&6.3E-07&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f5}}&$|W_{r,t}^{cner}|/N$&4.0E+05&2.6E-05&2.4E-05&2.5E-06&2.7E-06&4.0E-04&2.2E-04&4.0E-05&2.4E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&6.2E-06&6.2E-06&6.0E-07&8.0E-07&5.6E-04&2.6E-04&5.6E-05&2.9E-05&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f7}}&$|W_{r,t}^{cner}|/N$&4.0E+05&3.0E-05&4.3E-05&3.0E-06&4.8E-06&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&2.2E-05&1.1E-05&2.4E-06&1.5E-06&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f8}}&$|W_{r,t}^{cner}|/N$&4.0E+05&2.0E-06&2.4E-06&5.0E-07&1.0E-06&4.2E-05&3.3E-05&3.5E-06&3.0E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&6.0E-07&8.0E-07&0&0&3.7E-05&2.5E-05&5.2E-06&4.6E-06&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f9}}&$|W_{r,t}^{cner}|/N$&4.0E+05&6.0E-05&5.6E-05&5.5E-06&4.8E-06&3.1E-05&1.8E-05&4.0E-06&3.7E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&3.4E-06&3.1E-06&4.0E-07&8.0E-07&5.0E-06&3.6E-06&6.0E-07&8.0E-07&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f10}}&$|W_{r,t}^{cner}|/N$&7.9E+05&1.3E-05&8.1E-06&2.0E-06&1.3E-06&1.6E-04&2.4E-05&1.6E-05&2.7E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&3.6E-06&1.4E-06&6.0E-07&4.9E-07&3.4E-05&5.5E-06&2.8E-06&1.3E-06&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f12}}&$|W_{r,t}^{cner}|/N$&4.0E+05&3.5E-05&5.5E-05&3.0E-06&4.8E-06&2.2E-04&1.8E-04&1.7E-05&1.1E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.0E-05&1.0E-05&8.0E-07&1.6E-06&6.1E-04&6.0E-04&6.5E-05&6.3E-05&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f13}}&$|W_{r,t}^{cner}|/N$&4.0E+05&7.0E-06&6.0E-06&5.0E-07&1.0E-06&5.0E-04&3.9E-04&5.9E-05&4.5E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&2.2E-06&1.6E-06&4.0E-07&4.9E-07&2.1E-04&1.2E-04&2.3E-05&1.5E-05&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f14}}&$|W_{r,t}^{cner}|/N$&4.0E+05&3.2E-05&5.9E-05&0&0&3.2E-04&6.9E-05&3.4E-05&8.7E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&4.4E-06&4.6E-06&6.0E-07&1.2E-06&6.2E-05&1.5E-05&6.4E-06&2.7E-06&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f15}}&$|W_{r,t}^{cner}|/N$&4.0E+05&2.5E-05&2.5E-05&4.0E-06&3.4E-06&3.2E-04&2.7E-04&3.1E-05&2.1E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&2.4E-06&2.1E-06&4.0E-07&8.0E-07&4.8E-05&2.3E-05&4.4E-06&2.0E-06&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f16}}&$|W_{r,t}^{cner}|/N$&4.0E+05&5.7E-05&6.5E-05&5.0E-06&7.7E-06&4.1E-04&1.6E-04&3.5E-05&6.6E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&3.8E-06&5.3E-06&4.0E-07&8.0E-07&7.3E-05&3.1E-05&9.4E-06&5.2E-06&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f17}}&$|W_{r,t}^{cner}|/N$&6.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f18}}&$|W_{r,t}^{cner}|/N$&7.9E+05&5.2E-02&8.2E-03&4.0E-03&1.3E-03&2.6E-03&2.2E-03&2.6E-04&2.1E-04&1.9E-02&5.9E-03&2.5E-04&5.1E-04\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f19}}&$|W_{r,t}^{cner}|/N$&7.9E+05&2.8E-05&9.0E-06&4.6E-06&3.1E-06&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.0E-05&3.9E-06&1.2E-06&1.2E-06&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f20}}&$|W_{r,t}^{cner}|/N$&7.9E+05&3.3E-06&2.2E-06&5.1E-07&6.2E-07&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&3.6E-06&1.9E-06&8.0E-07&7.5E-07&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f21}}&$|W_{r,t}^{cner}|/N$&4.0E+05&2.1E-04&1.7E-04&2.1E-05&2.0E-05&8.0E-06&1.6E-05&1.0E-06&2.0E-06&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.8E-04&1.1E-04&2.2E-05&1.3E-05&9.4E-06&6.2E-06&8.0E-07&9.8E-07&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f22}}&$|W_{r,t}^{cner}|/N$&4.0E+05&2.3E-05&2.0E-05&1.0E-06&1.2E-06&1.3E-03&1.1E-04&1.2E-04&7.5E-05&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&2.0E-05&7.4E-06&2.2E-06&9.8E-07&1.3E-04&6.0E-05&1.1E-05&7.4E-06&0&0&0&0\\\cline{2-15}
		\hline
		
	
		
	\end{tabular}
	% 	}
\end{table}

 \begin{table}[htb!]
	% 	\resizebox{\columnwidth}{!}{%
	\scriptsize
	\centering
	\caption{\textcolor{red}{Sampling strategy: Sparse Grids, $\epsilon = 0$}
		\textcolor{blue}{--explain $\epsilon$, $t$, etc in caption; \textbf{bold} whats important?}} \label{tab:poles40}
	\setlength{\tabcolsep}{5pt}
	\begin{tabular}{|*{15}{c|}} 
		% 			{cc|c|c|c|c|c|c|c|c|c|c|c|c|}
		% 			\cline{3-15}
		% 			\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		% 			&\multicolumn{6}{|c|}{$\epsilon=0$}
		% 			&\multicolumn{6}{|c|}{$\epsilon=10^{-1}$}
		% 			\\
		\cline{4-15}
		\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\multicolumn{4}{|c|}{RA w/o Deg. Red.}
		&\multicolumn{4}{|c|}{RA w/ Deg. Red.}
		&\multicolumn{4}{|c|}{Pole Free RA}
		\\
		\cline{4-15}
		\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		\\
		\cline{1-15}
		\multicolumn{1}{|c|}{FNo.}
		&&\textit{N}&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		\\
		\cline{1-15}\hline\hline
		%		SG 0
		
		\multirow{2}{*}{\ref{fn:f1}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f2}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f3}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f4}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f5}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f7}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f8}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f9}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f10}}&$|W_{r,t}^{cner}|/N$&7.9E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f12}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f13}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f14}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f15}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f16}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f17}}&$|W_{r,t}^{cner}|/N$&6.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f18}}&$|W_{r,t}^{cner}|/N$&7.9E+05&5.3E-02&0&0&0&5.3E-02&0&0&0&5.4E-02&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f19}}&$|W_{r,t}^{cner}|/N$&7.9E+05&8.9E-06&0&8.9E-06&0&8.9E-06&0&8.9E-06&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f20}}&$|W_{r,t}^{cner}|/N$&7.9E+05&-1.3E-06&0&-1.3E-06&0&-1.3E-06&0&-1.3E-06&0&-1.3E-06&0&-1.3E-06&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&-1.0E-06&0&-1.0E-06&0&-1.0E-06&0&-1.0E-06&0&-1.0E-06&0&-1.0E-06&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f21}}&$|W_{r,t}^{cner}|/N$&4.0E+05&1.5E-05&0&0&0&1.5E-05&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.3E-04&0&1.0E-05&0&1.3E-04&0&1.0E-05&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f22}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		
		
		
	\end{tabular}
	% 	}
\end{table}

\begin{table}[htb!]
	% 	\resizebox{\columnwidth}{!}{%
	\scriptsize
	\centering
	\caption{\textcolor{red}{Sampling strategy: Sparse Grids, $\epsilon = 10^{-6}$}
		\textcolor{blue}{--explain $\epsilon$, $t$, etc in caption; \textbf{bold} whats important?}} \label{tab:poles41}
	\setlength{\tabcolsep}{5pt}
	\begin{tabular}{|*{15}{c|}} 
		% 			{cc|c|c|c|c|c|c|c|c|c|c|c|c|}
		% 			\cline{3-15}
		% 			\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		% 			&\multicolumn{6}{|c|}{$\epsilon=0$}
		% 			&\multicolumn{6}{|c|}{$\epsilon=10^{-1}$}
		% 			\\
		\cline{4-15}
		\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\multicolumn{4}{|c|}{RA w/o Deg. Red.}
		&\multicolumn{4}{|c|}{RA w/ Deg. Red.}
		&\multicolumn{4}{|c|}{Pole Free RA}
		\\
		\cline{4-15}
		\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		\\
		\cline{1-15}
		\multicolumn{1}{|c|}{FNo.}
		&&\textit{N}&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		\\
		\cline{1-15}\hline\hline
		%		SG 10-6
		
		\multirow{2}{*}{\ref{fn:f1}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f2}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f3}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f4}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f5}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f7}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f8}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&6.3E-05&0&7.5E-06&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&7.8E-05&0&1.1E-05&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f9}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f10}}&$|W_{r,t}^{cner}|/N$&7.9E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f12}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&5.9E-04&0&6.8E-05&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&1.3E-03&0&1.2E-04&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f13}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f14}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f15}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f16}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f17}}&$|W_{r,t}^{cner}|/N$&6.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f18}}&$|W_{r,t}^{cner}|/N$&7.9E+05&-1.3E-06&0&-1.3E-06&0&-1.3E-06&0&-1.3E-06&0&-1.3E-06&0&-1.3E-06&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&-1.0E-06&0&-1.0E-06&0&-1.0E-06&0&-1.0E-06&0&-1.0E-06&0&-1.0E-06&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f19}}&$|W_{r,t}^{cner}|/N$&7.9E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f20}}&$|W_{r,t}^{cner}|/N$&7.9E+05&-1.3E-06&0&-1.3E-06&0&-1.3E-06&0&-1.3E-06&0&-1.3E-06&0&-1.3E-06&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&-1.0E-06&0&-1.0E-06&0&-1.0E-06&0&-1.0E-06&0&-1.0E-06&0&-1.0E-06&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f21}}&$|W_{r,t}^{cner}|/N$&4.0E+05&1.5E-05&0&0&0&1.1E-04&0&1.0E-05&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.4E-04&0&9.0E-06&0&3.6E-05&0&4.0E-06&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f22}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		
		
		
	\end{tabular}
	% 	}
\end{table}

\begin{table}[htb!]
	% 	\resizebox{\columnwidth}{!}{%
	\scriptsize
	\centering
	\caption{\textcolor{red}{Sampling strategy: Sparse grids, $\epsilon = 10^{-2}$}
		\textcolor{blue}{--explain $\epsilon$, $t$, etc in caption; \textbf{bold} whats important?}} \label{tab:poles42}
	\setlength{\tabcolsep}{5pt}
	\begin{tabular}{|*{15}{c|}} 
		% 			{cc|c|c|c|c|c|c|c|c|c|c|c|c|}
		% 			\cline{3-15}
		% 			\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		% 			&\multicolumn{6}{|c|}{$\epsilon=0$}
		% 			&\multicolumn{6}{|c|}{$\epsilon=10^{-1}$}
		% 			\\
		\cline{4-15}
		\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\multicolumn{4}{|c|}{RA w/o Deg. Red.}
		&\multicolumn{4}{|c|}{RA w/ Deg. Red.}
		&\multicolumn{4}{|c|}{Pole Free RA}
		\\
		\cline{4-15}
		\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		&\multicolumn{2}{|c|}{$t=10^2$}
		&\multicolumn{2}{|c|}{$t=10^3$}
		\\
		\cline{1-15}
		\multicolumn{1}{|c|}{FNo.}
		&&\textit{N}&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		\\
		\cline{1-15}\hline\hline
		%		SG 10-2
		
		
		\multirow{2}{*}{\ref{fn:f1}}&$|W_{r,t}^{cner}|/N$&4.0E+05&2.5E-06&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&2.0E-06&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f2}}&$|W_{r,t}^{cner}|/N$&4.0E+05&1.7E-05&0&2.5E-06&0&1.6E-03&0&1.8E-04&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&4.0E-06&0&0&0&3.1E-03&0&3.0E-04&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f3}}&$|W_{r,t}^{cner}|/N$&4.0E+05&1.0E-05&0&0&0&8.0E-05&0&1.5E-05&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.1E-04&0&8.0E-06&0&3.7E-05&0&5.0E-06&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f4}}&$|W_{r,t}^{cner}|/N$&4.0E+05&3.5E-05&0&2.5E-06&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&2.3E-05&0&3.0E-06&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f5}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.3E-04&0&9.0E-06&0&5.4E-04&0&6.1E-05&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f7}}&$|W_{r,t}^{cner}|/N$&4.0E+05&3.5E-05&0&2.5E-06&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.6E-05&0&4.0E-06&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f8}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&3.0E-04&0&3.2E-05&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&3.8E-05&0&9.0E-06&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f9}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&1.5E-04&0&1.5E-05&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&1.0E-06&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f10}}&$|W_{r,t}^{cner}|/N$&7.9E+05&5.1E-06&0&1.3E-06&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.0E-06&0&0&0&2.0E-06&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f12}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&1.0E-03&0&1.4E-04&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&8.0E-06&0&0&0&1.3E-03&0&1.5E-04&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f13}}&$|W_{r,t}^{cner}|/N$&4.0E+05&5.0E-06&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.0E-06&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f14}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&3.1E-04&0&4.0E-05&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&5.0E-06&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f15}}&$|W_{r,t}^{cner}|/N$&4.0E+05&5.0E-06&0&0&0&7.5E-06&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&6.0E-06&0&1.0E-06&0&1.0E-06&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f16}}&$|W_{r,t}^{cner}|/N$&4.0E+05&0&0&0&0&4.3E-05&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&8.0E-06&0&1.0E-06&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f17}}&$|W_{r,t}^{cner}|/N$&6.0E+05&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&0&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f18}}&$|W_{r,t}^{cner}|/N$&7.9E+05&-1.3E-06&0&-1.3E-06&0&-1.3E-06&0&-1.3E-06&0&-1.3E-06&0&-1.3E-06&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&-1.0E-06&0&-1.0E-06&0&-1.0E-06&0&-1.0E-06&0&-1.0E-06&0&-1.0E-06&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f19}}&$|W_{r,t}^{cner}|/N$&7.9E+05&2.3E-05&0&1.3E-06&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&3.1E-05&0&0&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f20}}&$|W_{r,t}^{cner}|/N$&7.9E+05&-1.3E-06&0&-1.3E-06&0&-1.3E-06&0&-1.3E-06&0&-1.3E-06&0&-1.3E-06&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&-1.0E-06&0&-1.0E-06&0&-1.0E-06&0&-1.0E-06&0&-1.0E-06&0&-1.0E-06&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f21}}&$|W_{r,t}^{cner}|/N$&4.0E+05&2.8E-05&0&2.5E-06&0&3.5E-05&0&2.5E-06&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.5E-04&0&1.6E-05&0&6.0E-06&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		\multirow{2}{*}{\ref{fn:f22}}&$|W_{r,t}^{cner}|/N$&4.0E+05&1.7E-05&0&2.5E-06&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		&$|W_{r,t}^{in}|/N$&1.0E+06&1.4E-05&0&3.0E-06&0&0&0&0&0&0&0&0&0\\\cline{2-15}
		\hline
		
		
		
	\end{tabular}
	% 	}
\end{table}
\clearpage

%###################################################

\begin{figure}[htb!]
	\centering
	\resizebox{\textwidth}{6in}{
		\input{images/tmpimages/Perrorbars_for_lhs.pgf}
	}
	\caption{errors for Sampling strategy: Latin hypercube sampling. $\epsilon = 0$ (top), $\epsilon = 10^{-1}$ (middle), $\epsilon = 10^{-3}$ (bottom)
%		Comparison of testing error $\Delta_r$ between the polynomial and rational approximations over noise-free (left) and noisy (right) interpolation data with $\epsilon=10^{-1}$ noise
}
	\label{fig:errorbarplot}
\end{figure}

\begin{figure}[htb!]
	\centering
	\resizebox{\textwidth}{6in}{
		\input{images/tmpimages/Perrorbars_for_mc.pgf}
	}
	\caption{errors for Sampling strategy: Uniform random. $\epsilon = 0$ (top), $\epsilon = 10^{-1}$ (middle), $\epsilon = 10^{-3}$ (bottom)}
	\label{fig:errorbarplot1}
\end{figure}

\begin{figure}[htb!]
	\centering
	\resizebox{\textwidth}{6in}{
		\input{images/tmpimages/Perrorbars_for_so.pgf}
	}
	\caption{errors for Sampling strategy: Sobol sequence sampling. $\epsilon = 0$ (top), $\epsilon = 10^{-1}$ (middle), $\epsilon = 10^{-3}$ (bottom)}
	\label{fig:errorbarplot2}
\end{figure}

\begin{figure}[htb!]
	\centering
	\resizebox{\textwidth}{6in}{
		\input{images/tmpimages/Perrorbars_for_sg.pgf}
	}
	\caption{errors for Sampling strategy: Sparse Grids. $\epsilon = 0$ (top), $\epsilon = 10^{-1}$ (middle), $\epsilon = 10^{-3}$ (bottom)}
	\label{fig:errorbarplot3}
\end{figure}

\begin{figure}[htb!]
	\centering
	\resizebox{\textwidth}{6in}{
		\input{images/tmpimages/Perrorbars_for_0.pgf}
	}
	\caption{errors for Noise level $\epsilon = 0$. }
	\label{fig:errorbarplot4}
\end{figure}

\begin{figure}[htb!]
	\centering
	\resizebox{\textwidth}{6in}{
		\input{images/tmpimages/Perrorbars_for_10-2.pgf}
	}
	\caption{errors for Noise level $\epsilon = 10^{-2}$.}
	\label{fig:errorbarplot5}
\end{figure}

\begin{figure}[htb!]
	\centering
	\resizebox{\textwidth}{6in}{
		\input{images/tmpimages/Perrorbars_for_10-6.pgf}
	}
	\caption{errors for Noise level $\epsilon = 10^{-6}$. }
	\label{fig:errorbarplot6}
\end{figure}


%###################################################
\clearpage
\begin{figure}[htb!]
	\centering
	\begin{subfigure}[b]{0.28\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/fndiffPA.png}
		\caption{Polynomial Approximation}    
		\label{fig:fndiffpa}
	\end{subfigure}
%	\hfill
	\begin{subfigure}[b]{0.28\textwidth}  
		\centering
		\includegraphics[width=\textwidth]{images/fndiffRA.png}
		\caption{Algorithm~\ref{ALG:MVVandQR}}    
		\label{fig:fndiffra}
	\end{subfigure}
%	\vskip\baselineskip
	\begin{subfigure}[b]{0.28\textwidth}  
		\centering
		\includegraphics[width=\textwidth]{images/fndiffRASIP.png}
		\caption{Algorithm~\ref{A:Polyak}}    
		\label{fig:fndiffrasip}
	\end{subfigure}
	\begin{subfigure}[b]{0.1\textwidth}  
		\centering
		\includegraphics[width=.55\textwidth]{images/fndiffCB.png}
	\end{subfigure}
	\caption{$\Delta_r$ obtained for noise-free interpolation data of~\ref{fn:f8} \mohan{todo}{figure incorrect. update}}
	\label{fig:fndiff}
\end{figure}

The testing error obtained for the polynomial and the two rational approximations over noise-free  and noisy interpolation data of functions from \cref{T:TPs} is shown in \cref{fig:errorbarplot} and the testing error obtained by the approximations is illustrated using a surface plot in \cref{fig:fndiff}. 
The order of the polynomials are chosen such that the rational approximation using Algorithm~\ref{ALG:MVVandQR} has no poles. 
Also, the degrees of freedom in the polynomial approximation is at least as much as that of the two rational approximations.
It is observed that in the noise-free case, the rational approximations fit the rational functions of~\ref{fn:f8}, \ref{fn:f13}, and \ref{fn:f14} much better than the other functions, which can be approximated using Taylor series expansions. 
Furthermore, the rational approximation using Algorithm~\ref{ALG:MVVandQR} outperforms the one using Algorithm~\ref{A:Polyak}. \textcolor{blue}{I dont understand this sentence: }However, this performance gain is when the errors are really low for both approaches, which is less significant than when the performance gain is the other way around for errors that are greater than one.
 When noise is introduced in the interpolation data, the results are similar to those observed in \cref{tab:poles}. Additionally, the testing error obtained from the rational approximation using Algorithm~\ref{A:Polyak} is better than the polynomial approximation unless the interpolation data is from the polynomial function of~\ref{fn:f22}, in which case, the testing errors are closer. 

\mohan{Remark/Question}{Sven and Anthony: Please check and correct the paragraph below} 

In \cref{fig:errorbarplot}, we see that over noise-free interpolation points of rational functions~\ref{fn:f8}, \ref{fn:f13}, and \ref{fn:f14}, the rational approximation using Algorithm~\ref{ALG:MVVandQR} gives much better testing error than  Algorithm~\ref{A:Polyak}. This difference in testing error is because Algorithm~\ref{ALG:MVVandQR} performs the approximation using multivariate \textit{Stieltjes} process whereas Algorithm~\ref{A:Polyak} performs the approximation using optimization over functions in monomial basis.

%%% ========================================================================== %%%
\subsection{Computational Effort of Computing Approximations}
\textcolor{blue}{I have a hard time parsing this section}
In this section, we delve deeper into the performance of rational approximation using Algorithm~\ref{A:Polyak} and then compare the computational effort required to compute all three approximations. 
\cref{fig:algostatsplot} shows the time taken and the solutions \textcolor{blue}{what are the ``solutions''?} obtained from solving the fitting problem in \eqref{eq:rationalApproxFD} and the problem of (global) minimization of $q_l(x)$ across 1418 iterations of Algorithm~\ref{A:Polyak}. 
The function being approximated is~\ref{fn:f20} with seven variables and the approximation has 366 degrees of freedom. 
The solution of the fitting problem increases as more constraints are added to remove poles while the time taken to solve this problem shows little difference. 
On the other hand, the solution of the (global) minimization problem increases as more constraints are added to the fitting problem. The time taken to solve this problem increases towards the end as more multistarts are required to find regions where $q_l(x) \le0$.
Additionally, large number of iterations are required to find an approximation without poles because of the degrees of freedom considered in the approximation and since only one constraint is added to the fitting problem in each iteration. 
When the approximations are performed for a wide range of numerator and denominator polynomial orders, we found that the time and number of iterations are more sensitive to the order of the denominator polynomial $N$ as shown in \cref{fig:algostatsplot}. More specifically, the fit time increases very gradually with $N$, whereas the total time is influenced more by the multistart time. 


\begin{figure}[htb!]
	\centering
	\includegraphics[width=.7\textwidth]{images/iterationinfo.pdf}
	\caption{Solutions and time taken per iteration from solving the fitting problem (top) and (global) minimization problem (bottom) in Algorithm~\ref{A:Polyak}.}
	\label{fig:iterationstatsplot}
\end{figure}

\begin{figure}[htb!]
	\centering
	\includegraphics[width=1\textwidth]{images/algorithmstats.pdf}
	\caption{Distribution of time and number of iterations for rational approximations using Algorithm~\ref{A:Polyak} over~all $n=2$ functions from Table~\ref{T:TPs}.}
	\label{fig:algostatsplot}
\end{figure}

\cref{tab:cputimes} shows the total CPU time taken by the three approximation approaches with noise-free and noisy interpolation data. As the degrees of freedom increase, the CPU times for the rational approximation using Algorithm~\ref{A:Polyak} increases almost exponentially. Contributors of this are the number of iterations completed by Algorithm~\ref{A:Polyak} and the number of multistart performed in each iteration as a function of the number of nonlinearities (\textit{nnl}) in the denominator polynomial using~\eqref{eq:multistart}  to solve the (global) minimization problem. On the other hand, the other two approximations grow more slowly with the degrees of freedom. When noise is added to the interpolation data, the number of iterations required to remove the poles is more for a number of functions and this contributes to even higher run times with Algorithm~\ref{A:Polyak}. Despite this, the run time of Algorithm~\ref{A:Polyak} for three functions namely,~\ref{fn:f3}, \ref{fn:f14} and \ref{fn:f21} are better than that of Algorithm~\ref{ALG:MVVandQR}. 

%###################################################
%TODO
%Same table as below for different sampling stratefies (*4)

\clearpage
 \begin{table}[htb!]
	% 	\resizebox{\columnwidth}{!}{%
	\tiny
	\centering
	\caption{Total CPU time in seconds taken by rational and polynomial approximation approaches where the interpolation points are selected using \textbf{uniform random sampling}} \label{tab:cputimes}
	\setlength{\tabcolsep}{2pt}
	\begin{tabular}{|*{34}{c|}} 
		% 			{cc|c|c|c|c|c|c|c|c|c|c|c|c|}
		\cline{5-34}
		\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\multicolumn{10}{|c|}{$\epsilon=0$}
		&\multicolumn{10}{|c|}{$\epsilon=10^{-2}$}
		&\multicolumn{10}{|c|}{$\epsilon=10^{-6}$}
		\\
		\cline{1-34}
		FNo.
		&\makecell{\textit{DoF}\\ for \\poly.\\approx.}
		&\makecell{\textit{DoF}\\ for\\ rational\\approx.}
		&\makecell{\textit{nnl}\\ in \\$q(x)$}
		& \multicolumn{2}{|c|}{\makecell{Poly.\\approx.}}
		& \multicolumn{2}{|c|}{\makecell{Algorithm\\ RA}}
		& \multicolumn{2}{|c|}{\makecell{Algorithm\\ RA with DR}}
		& \multicolumn{4}{|c|}{\makecell{Algorithm\\ ~\ref{A:Polyak}}}
		& \multicolumn{2}{|c|}{\makecell{Poly.\\approx.}}
		& \multicolumn{2}{|c|}{\makecell{Algorithm\\ RA}}
		& \multicolumn{2}{|c|}{\makecell{Algorithm\\ RA with DR}}
		& \multicolumn{4}{|c|}{\makecell{Algorithm\\ ~\ref{A:Polyak}}}
		& \multicolumn{2}{|c|}{\makecell{Poly.\\approx.}}
		& \multicolumn{2}{|c|}{\makecell{Algorithm\\ RA}}
		& \multicolumn{2}{|c|}{\makecell{Algorithm\\ RA with DR}}
		& \multicolumn{4}{|c|}{\makecell{Algorithm\\ ~\ref{A:Polyak}}}
		\\
		\cline{1-34}
		\multicolumn{1}{|c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		& \multicolumn{2}{|c|}{\makecell{iterations}}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		& \multicolumn{2}{|c|}{\makecell{iterations}}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		& \multicolumn{2}{|c|}{\makecell{iterations}}
		\\
		\cline{1-34}
		\multicolumn{1}{|c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}
		\\
		\hline\hline
		
		\ref{fn:f1}&45&42&18&0.9&0.0&3.9&0.0&3.6&0.1&45.3&0.1&1.0&0.0&0.9&0.0&3.9&0.0&3.9&0.0&41.1&0.4&1.2&0.4&0.9&0.0&3.6&0.0&3.6&0.0&30.8&0.7&1.0&0.0\\\hline
		\ref{fn:f2}&45&42&18&0.9&0.0&3.9&0.0&3.6&0.0&45.2&0.1&1.0&0.0&0.9&0.0&3.9&0.0&3.9&0.0&40.4&0.0&1.0&0.0&0.9&0.0&3.7&0.0&3.7&0.1&30.1&1.2&1.0&0.0\\\hline
		\ref{fn:f3}&45&42&18&0.9&0.0&3.9&0.0&3.7&0.1&43.8&0.2&1.0&0.0&0.9&0.0&3.9&0.0&3.9&0.0&40.4&0.2&1.0&0.0&0.8&0.0&3.8&0.0&3.8&0.0&29.1&0.9&1.0&0.0\\\hline
		\ref{fn:f4}&45&42&18&0.8&0.0&3.9&0.1&3.8&0.1&45.2&0.1&1.0&0.0&0.9&0.0&3.8&0.1&3.9&0.1&43.0&0.1&1.0&0.0&0.9&0.0&3.8&0.1&3.8&0.1&30.2&0.0&1.0&0.0\\\hline
		\ref{fn:f5}&45&42&18&0.9&0.0&3.7&0.0&3.8&0.0&43.7&0.1&1.0&0.0&0.9&0.0&3.7&0.0&3.8&0.0&40.5&0.1&1.0&0.0&0.9&0.0&3.8&0.0&3.8&0.0&29.5&0.5&1.0&0.0\\\hline
		\ref{fn:f7}&45&42&18&0.9&0.1&3.5&0.5&3.6&0.5&43.8&0.1&1.0&0.0&0.8&0.1&3.5&0.5&3.5&0.5&40.4&0.1&1.0&0.0&0.8&0.1&3.6&0.5&3.6&0.5&27.5&2.0&1.0&0.0\\\hline
		\ref{fn:f8}&45&42&18&0.7&0.0&2.4&0.1&2.5&0.1&45.1&0.2&1.8&1.0&0.7&0.0&2.4&0.1&2.5&0.1&41.2&0.2&1.8&1.2&0.7&0.0&2.5&0.1&2.5&0.1&29.9&1.1&2.4&1.0\\\hline
		\ref{fn:f9}&45&42&18&0.7&0.0&2.4&0.4&2.6&0.3&45.3&0.1&1.0&0.0&0.7&0.0&2.4&0.4&2.5&0.3&40.1&0.4&1.0&0.0&0.7&0.0&2.5&0.4&2.6&0.3&30.3&1.1&1.0&0.0\\\hline
		\ref{fn:f10}&330&252&121&0.7&0.0&3.0&0.0&3.1&0.0&420.2&8.1&3.2&2.2&0.7&0.0&3.0&0.0&3.2&0.0&407.2&1.7&1.8&0.4&0.7&0.0&3.1&0.0&3.2&0.0&685.0&247.9&4.8&3.5\\\hline
		\ref{fn:f12}&45&42&18&0.7&0.0&2.3&0.0&2.3&0.0&44.3&0.1&1.0&0.0&0.7&0.0&2.2&0.0&2.3&0.1&38.7&0.1&1.0&0.0&0.6&0.0&2.3&0.0&2.3&0.0&27.9&1.3&1.0&0.0\\\hline
		\ref{fn:f13}&45&42&18&0.6&0.0&2.3&0.0&2.3&0.0&43.9&0.2&1.0&0.0&0.7&0.0&2.2&0.0&2.3&0.0&38.8&0.2&1.0&0.0&0.7&0.0&2.3&0.0&2.3&0.0&27.0&1.3&1.0&0.0\\\hline
		\ref{fn:f14}&45&42&18&0.6&0.0&2.3&0.0&2.3&0.0&45.0&0.1&1.0&0.0&0.7&0.0&2.2&0.0&2.3&0.0&39.6&0.1&1.0&0.0&0.7&0.0&2.3&0.0&2.3&0.0&28.6&1.9&1.0&0.0\\\hline
		\ref{fn:f15}&45&42&18&0.5&0.1&3.2&0.6&2.8&0.3&44.9&0.1&1.0&0.0&0.8&0.1&3.1&0.6&3.2&0.6&39.1&0.4&1.0&0.0&0.7&0.1&2.8&0.4&2.9&0.4&30.9&0.2&1.0&0.0\\\hline
		\ref{fn:f16}&45&42&18&0.4&0.0&3.9&0.0&3.1&0.0&44.7&0.5&1.0&0.0&0.9&0.0&3.7&0.0&3.9&0.0&40.2&0.2&1.0&0.0&0.9&0.0&3.2&0.0&3.2&0.0&30.5&0.5&1.0&0.0\\\hline
		\ref{fn:f17}&120&112&52&0.4&0.0&4.0&0.0&3.2&0.0&76.0&2.9&2.8&1.8&0.9&0.0&3.8&0.0&4.1&0.0&74.5&2.1&3.6&1.4&0.8&0.0&3.4&0.1&3.4&0.0&62.5&3.4&3.0&2.2\\\hline
		\ref{fn:f18}&330&252&121&0.5&0.0&4.7&0.0&4.1&0.2&520.1&13.5&22.6&3.1&0.9&0.0&4.4&0.0&4.9&0.0&512.2&13.5&24.2&2.9&0.8&0.0&4.1&0.1&4.1&0.1&515.6&8.0&23.6&2.2\\\hline
		\ref{fn:f19}&330&252&121&0.5&0.0&4.7&0.0&4.3&0.0&413.3&0.5&1.0&0.0&0.9&0.0&4.4&0.0&4.8&0.0&409.5&0.8&1.0&0.0&0.8&0.0&4.3&0.0&4.2&0.0&399.3&0.4&1.0&0.0\\\hline
		\ref{fn:f20}&330&252&121&0.5&0.0&4.7&0.0&4.3&0.0&825.9&186.7&73.6&27.2&0.9&0.0&4.4&0.0&4.8&0.0&704.3&115.5&71.8&26.8&0.7&0.0&4.4&0.0&4.4&0.0&835.4&130.5&77.4&28.4\\\hline
		\ref{fn:f21}&45&42&18&0.5&0.0&2.9&0.7&2.7&0.6&43.8&0.1&1.2&0.4&0.8&0.1&2.6&0.7&2.9&0.7&40.4&0.1&1.2&0.4&0.6&0.1&2.8&0.7&2.7&0.6&29.0&1.6&1.2&0.4\\\hline
		\ref{fn:f22}&45&42&18&0.5&0.0&2.4&0.4&2.4&0.3&44.9&1.2&1.0&0.0&0.7&0.1&2.3&0.4&2.5&0.4&40.4&0.1&1.0&0.0&0.5&0.0&2.4&0.4&2.4&0.3&29.8&0.9&1.0&0.0\\\hline

	\end{tabular}
	% 	}
\end{table}


 \begin{table}[htb!]
	% 	\resizebox{\columnwidth}{!}{%
	\tiny
	\centering
	\caption{Total CPU time in seconds taken by rational and polynomial approximation approaches where the interpolation points are selected using \textbf{LHS}} \label{tab:cputimes1}
	\setlength{\tabcolsep}{2pt}
	\begin{tabular}{|*{34}{c|}} 
		% 			{cc|c|c|c|c|c|c|c|c|c|c|c|c|}
		\cline{5-34}
		\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\multicolumn{10}{|c|}{$\epsilon=0$}
		&\multicolumn{10}{|c|}{$\epsilon=10^{-2}$}
		&\multicolumn{10}{|c|}{$\epsilon=10^{-6}$}
		\\
		\cline{1-34}
		FNo.
		&\makecell{\textit{DoF}\\ for \\poly.\\approx.}
		&\makecell{\textit{DoF}\\ for\\ rational\\approx.}
		&\makecell{\textit{nnl}\\ in \\$q(x)$}
		& \multicolumn{2}{|c|}{\makecell{Poly.\\approx.}}
		& \multicolumn{2}{|c|}{\makecell{Algorithm\\ RA}}
		& \multicolumn{2}{|c|}{\makecell{Algorithm\\ RA with DR}}
		& \multicolumn{4}{|c|}{\makecell{Algorithm\\ ~\ref{A:Polyak}}}
		& \multicolumn{2}{|c|}{\makecell{Poly.\\approx.}}
		& \multicolumn{2}{|c|}{\makecell{Algorithm\\ RA}}
		& \multicolumn{2}{|c|}{\makecell{Algorithm\\ RA with DR}}
		& \multicolumn{4}{|c|}{\makecell{Algorithm\\ ~\ref{A:Polyak}}}
		& \multicolumn{2}{|c|}{\makecell{Poly.\\approx.}}
		& \multicolumn{2}{|c|}{\makecell{Algorithm\\ RA}}
		& \multicolumn{2}{|c|}{\makecell{Algorithm\\ RA with DR}}
		& \multicolumn{4}{|c|}{\makecell{Algorithm\\ ~\ref{A:Polyak}}}
		\\
		\cline{1-34}
		\multicolumn{1}{|c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		& \multicolumn{2}{|c|}{\makecell{iterations}}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		& \multicolumn{2}{|c|}{\makecell{iterations}}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		& \multicolumn{2}{|c|}{\makecell{iterations}}
		\\
		\cline{1-34}
		\multicolumn{1}{|c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}
		\\
		\hline\hline
		
		\ref{fn:f1}&45&42&18&0.8&0.0&4.0&0.0&3.4&0.1&37.4&0.2&1.0&0.0&0.9&0.0&4.0&0.0&3.9&0.0&28.9&1.5&1.4&0.5&1.0&0.1&3.3&0.1&4.2&0.0&30.7&0.2&1.0&0.0\\\hline
		\ref{fn:f2}&45&42&18&0.8&0.0&4.0&0.0&3.5&0.1&37.7&0.3&1.0&0.0&0.9&0.0&4.0&0.0&3.9&0.0&29.5&0.3&1.0&0.0&0.9&0.0&3.4&0.1&4.2&0.0&31.1&0.1&1.0&0.0\\\hline
		\ref{fn:f3}&45&42&18&0.8&0.0&4.0&0.0&3.9&0.1&36.2&0.2&1.0&0.0&0.9&0.0&4.0&0.0&3.9&0.0&30.3&0.6&2.4&0.5&0.9&0.0&3.6&0.1&4.2&0.0&29.8&0.0&1.0&0.0\\\hline
		\ref{fn:f4}&45&42&18&0.8&0.0&4.0&0.1&3.9&0.1&37.9&0.1&1.0&0.0&0.9&0.0&4.0&0.1&3.9&0.1&32.2&0.2&1.0&0.0&0.9&0.0&3.7&0.1&4.1&0.1&30.4&0.2&1.0&0.0\\\hline
		\ref{fn:f5}&45&42&18&0.8&0.0&3.9&0.0&3.8&0.0&36.2&0.2&1.0&0.0&1.0&0.0&3.9&0.0&3.8&0.0&29.8&0.1&1.0&0.0&0.9&0.0&3.7&0.1&4.1&0.0&29.8&0.1&1.0&0.0\\\hline
		\ref{fn:f7}&45&42&18&0.8&0.1&3.6&0.6&3.5&0.5&36.5&0.3&1.0&0.0&0.9&0.1&3.6&0.5&3.6&0.5&29.9&0.2&1.0&0.0&0.9&0.1&3.4&0.4&3.8&0.6&29.7&0.2&1.0&0.0\\\hline
		\ref{fn:f8}&45&42&18&0.6&0.0&2.5&0.0&2.5&0.1&37.3&0.3&2.0&0.6&0.7&0.0&2.5&0.0&2.5&0.1&30.3&0.5&2.2&0.4&0.7&0.0&2.5&0.1&2.6&0.0&28.7&1.2&2.4&1.7\\\hline
		\ref{fn:f9}&45&42&18&0.6&0.1&2.6&0.3&2.5&0.3&37.9&0.2&1.2&0.4&0.7&0.0&2.6&0.3&2.5&0.3&28.2&1.4&3.4&0.8&0.7&0.0&2.5&0.3&2.7&0.4&29.4&1.0&1.0&0.0\\\hline
		\ref{fn:f10}&330&252&121&0.6&0.0&3.2&0.0&3.1&0.0&403.1&12.3&3.8&2.0&0.7&0.0&3.1&0.0&3.2&0.0&399.8&6.0&2.6&1.4&0.7&0.0&3.2&0.0&3.4&0.0&462.2&58.2&2.8&1.9\\\hline
		\ref{fn:f12}&45&42&18&0.6&0.0&2.5&0.0&2.3&0.0&36.9&0.3&1.0&0.0&0.7&0.0&2.4&0.0&2.4&0.0&26.7&0.2&1.0&0.0&0.7&0.0&2.4&0.1&2.6&0.0&28.3&0.4&1.0&0.0\\\hline
		\ref{fn:f13}&45&42&18&0.6&0.0&2.5&0.0&2.3&0.0&44.7&16.2&1.0&0.0&0.7&0.0&2.4&0.0&2.4&0.0&26.8&0.3&1.0&0.0&0.6&0.0&2.4&0.0&2.6&0.0&27.7&0.7&1.0&0.0\\\hline
		\ref{fn:f14}&45&42&18&0.6&0.0&2.5&0.0&2.3&0.0&37.5&0.3&1.0&0.0&0.6&0.0&2.4&0.0&2.4&0.0&27.2&0.4&1.0&0.0&0.6&0.0&2.3&0.1&2.5&0.0&28.9&0.3&1.0&0.0\\\hline
		\ref{fn:f15}&45&42&18&0.7&0.1&3.3&0.7&2.8&0.3&37.6&0.3&1.0&0.0&0.6&0.1&3.3&0.7&3.2&0.6&29.3&1.3&1.0&0.0&0.5&0.1&2.5&0.2&3.4&0.7&29.1&0.1&1.0&0.0\\\hline
		\ref{fn:f16}&45&42&18&0.8&0.0&4.0&0.0&3.0&0.0&37.4&0.5&1.0&0.0&0.5&0.0&4.0&0.0&3.9&0.0&29.6&0.2&1.0&0.0&0.4&0.0&2.5&0.0&4.2&0.0&30.4&0.9&1.0&0.0\\\hline
		\ref{fn:f17}&120&112&52&0.8&0.0&4.2&0.0&3.2&0.1&67.4&1.1&1.8&0.7&0.5&0.0&4.1&0.0&4.1&0.0&63.4&1.4&3.4&1.0&0.4&0.0&2.7&0.1&4.3&0.0&63.1&2.5&3.0&1.7\\\hline
		\ref{fn:f18}&330&252&121&0.8&0.0&4.8&0.0&4.0&0.2&519.5&22.7&30.2&5.0&0.6&0.1&4.8&0.1&4.8&0.0&530.5&25.7&29.6&3.0&0.5&0.0&3.5&0.1&5.0&0.1&515.4&16.6&28.4&4.2\\\hline
		\ref{fn:f19}&330&252&121&0.8&0.0&4.8&0.0&4.2&0.0&386.2&0.4&1.0&0.0&0.7&0.0&4.8&0.0&4.8&0.0&402.0&5.6&1.4&0.8&0.5&0.0&3.7&0.0&5.0&0.0&398.2&2.0&1.0&0.0\\\hline
		\ref{fn:f20}&330&252&121&0.7&0.0&4.7&0.0&4.3&0.0&471.2&33.7&23.2&9.6&0.7&0.0&4.8&0.0&4.8&0.0&502.8&43.5&24.8&9.1&0.6&0.0&3.8&0.0&5.1&0.0&490.6&35.5&24.8&8.7\\\hline
		\ref{fn:f21}&45&42&18&0.5&0.1&2.8&0.7&2.7&0.6&37.2&0.8&1.2&0.4&0.6&0.1&3.0&0.7&2.9&0.7&30.0&0.3&1.2&0.4&0.5&0.0&2.5&0.4&3.2&0.7&30.5&1.0&1.2&0.4\\\hline
		\ref{fn:f22}&45&42&18&0.5&0.1&2.4&0.4&2.4&0.3&42.3&10.6&1.0&0.0&0.6&0.1&2.5&0.3&2.6&0.3&29.4&0.2&1.0&0.0&0.5&0.0&2.3&0.3&2.7&0.4&30.6&0.7&1.0&0.0\\\hline
		
	\end{tabular}
	% 	}
\end{table}

 \begin{table}[htb!]
	% 	\resizebox{\columnwidth}{!}{%
	\tiny
	\centering
	\caption{Total CPU time in seconds taken by rational and polynomial approximation approaches where the interpolation points are selected using \textbf{Sobol} sampling} \label{tab:cputimes2}
	\setlength{\tabcolsep}{2pt}
	\begin{tabular}{|*{34}{c|}} 
		% 			{cc|c|c|c|c|c|c|c|c|c|c|c|c|}
		\cline{5-34}
		\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\multicolumn{10}{|c|}{$\epsilon=0$}
		&\multicolumn{10}{|c|}{$\epsilon=10^{-2}$}
		&\multicolumn{10}{|c|}{$\epsilon=10^{-6}$}
		\\
		\cline{1-34}
		FNo.
		&\makecell{\textit{DoF}\\ for \\poly.\\approx.}
		&\makecell{\textit{DoF}\\ for\\ rational\\approx.}
		&\makecell{\textit{nnl}\\ in \\$q(x)$}
		& \multicolumn{2}{|c|}{\makecell{Poly.\\approx.}}
		& \multicolumn{2}{|c|}{\makecell{Algorithm\\ RA}}
		& \multicolumn{2}{|c|}{\makecell{Algorithm\\ RA with DR}}
		& \multicolumn{4}{|c|}{\makecell{Algorithm\\ ~\ref{A:Polyak}}}
		& \multicolumn{2}{|c|}{\makecell{Poly.\\approx.}}
		& \multicolumn{2}{|c|}{\makecell{Algorithm\\ RA}}
		& \multicolumn{2}{|c|}{\makecell{Algorithm\\ RA with DR}}
		& \multicolumn{4}{|c|}{\makecell{Algorithm\\ ~\ref{A:Polyak}}}
		& \multicolumn{2}{|c|}{\makecell{Poly.\\approx.}}
		& \multicolumn{2}{|c|}{\makecell{Algorithm\\ RA}}
		& \multicolumn{2}{|c|}{\makecell{Algorithm\\ RA with DR}}
		& \multicolumn{4}{|c|}{\makecell{Algorithm\\ ~\ref{A:Polyak}}}
		\\
		\cline{1-34}
		\multicolumn{1}{|c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		& \multicolumn{2}{|c|}{\makecell{iterations}}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		& \multicolumn{2}{|c|}{\makecell{iterations}}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		& \multicolumn{2}{|c|}{\makecell{iterations}}
		\\
		\cline{1-34}
		\multicolumn{1}{|c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}
		\\
		\hline\hline
		
		\ref{fn:f1}&45&42&18&0.9&0.0&3.9&0.0&3.9&0.0&39.2&0.3&1.0&0.0&0.8&0.0&4.0&0.0&3.6&0.1&29.7&2.1&2.0&0.6&0.9&0.0&3.9&0.0&3.9&0.0&35.4&0.3&1.0&0.0\\\hline
		\ref{fn:f2}&45&42&18&0.9&0.0&3.9&0.0&3.9&0.0&39.2&0.2&1.0&0.0&0.8&0.0&4.0&0.0&3.6&0.1&31.0&0.1&1.0&0.0&0.9&0.0&3.9&0.0&3.9&0.0&35.2&0.2&1.0&0.0\\\hline
		\ref{fn:f3}&45&42&18&0.9&0.0&3.9&0.0&3.9&0.0&37.7&0.3&1.0&0.0&0.8&0.0&4.0&0.0&3.8&0.0&31.5&0.4&2.0&0.9&0.9&0.0&3.9&0.0&3.9&0.0&33.9&0.4&1.0&0.0\\\hline
		\ref{fn:f4}&45&42&18&0.8&0.0&3.9&0.1&3.9&0.1&39.1&0.0&1.0&0.0&0.8&0.0&3.9&0.1&3.8&0.1&33.5&0.1&1.0&0.0&0.9&0.0&3.8&0.1&3.8&0.1&34.5&0.3&1.0&0.0\\\hline
		\ref{fn:f5}&45&42&18&0.9&0.0&3.8&0.0&3.8&0.0&35.3&2.2&1.0&0.0&0.8&0.0&3.9&0.0&3.8&0.0&30.8&0.1&1.0&0.0&0.8&0.1&3.8&0.0&3.8&0.0&33.8&0.2&1.0&0.0\\\hline
		\ref{fn:f7}&45&42&18&0.8&0.1&3.5&0.6&3.5&0.5&38.0&0.2&1.0&0.0&0.8&0.1&3.6&0.5&3.6&0.5&29.4&1.7&1.0&0.0&0.7&0.1&3.5&0.5&3.6&0.5&34.2&0.1&1.0&0.0\\\hline
		\ref{fn:f8}&45&42&18&0.6&0.0&2.4&0.1&2.4&0.1&39.2&0.3&1.6&0.8&0.6&0.0&2.5&0.0&2.5&0.1&28.3&1.7&2.4&0.8&0.5&0.0&2.4&0.0&2.5&0.1&35.4&0.7&2.6&1.2\\\hline
		\ref{fn:f9}&45&42&18&0.7&0.1&2.5&0.4&2.5&0.3&39.6&0.1&1.0&0.0&0.6&0.1&2.6&0.4&2.5&0.3&30.7&1.3&2.2&1.2&0.6&0.1&2.5&0.4&2.6&0.3&33.3&1.1&1.2&0.4\\\hline
		\ref{fn:f10}&330&252&121&0.7&0.0&3.1&0.0&3.1&0.1&427.0&7.8&4.0&1.8&0.6&0.0&3.2&0.0&3.2&0.0&404.8&9.7&2.4&0.8&0.6&0.0&3.0&0.0&3.2&0.0&447.3&59.0&2.2&1.5\\\hline
		\ref{fn:f12}&45&42&18&0.6&0.0&2.3&0.0&2.3&0.0&36.0&1.8&1.0&0.0&0.6&0.0&2.5&0.0&2.3&0.0&30.9&0.2&1.0&0.0&0.5&0.0&2.3&0.0&2.3&0.1&32.6&1.2&1.0&0.0\\\hline
		\ref{fn:f13}&45&42&18&0.6&0.0&2.3&0.1&2.3&0.1&35.3&2.0&1.0&0.0&0.6&0.0&2.4&0.0&2.3&0.0&28.0&1.6&1.0&0.0&0.5&0.0&2.3&0.1&2.3&0.0&34.3&0.1&1.0&0.0\\\hline
		\ref{fn:f14}&45&42&18&0.6&0.0&2.3&0.0&2.3&0.1&35.6&1.7&1.0&0.0&0.6&0.0&2.5&0.0&2.3&0.0&29.8&1.1&1.0&0.0&0.5&0.0&2.3&0.0&2.4&0.0&35.2&0.1&1.0&0.0\\\hline
		\ref{fn:f15}&45&42&18&0.7&0.1&3.2&0.6&3.2&0.7&39.2&0.1&1.0&0.0&0.7&0.1&3.3&0.7&2.9&0.3&30.3&1.6&1.0&0.0&0.6&0.1&3.2&0.7&3.3&0.6&35.0&0.2&1.0&0.0\\\hline
		\ref{fn:f16}&45&42&18&0.9&0.0&3.9&0.0&3.9&0.0&39.2&0.1&1.0&0.0&0.8&0.0&4.0&0.0&3.2&0.1&30.9&0.2&1.0&0.0&0.5&0.0&3.9&0.0&3.9&0.0&33.8&1.3&1.0&0.0\\\hline
		\ref{fn:f17}&120&112&52&0.9&0.0&4.0&0.0&4.0&0.0&71.4&4.3&3.2&2.9&0.8&0.0&4.1&0.0&3.4&0.1&63.5&1.4&2.6&1.0&0.5&0.0&4.0&0.0&4.1&0.0&67.4&4.3&3.2&3.1\\\hline
		\ref{fn:f18}&330&252&121&0.9&0.0&4.7&0.0&4.7&0.1&526.1&19.7&27.0&5.2&0.9&0.0&4.8&0.0&4.2&0.1&534.7&47.8&31.2&4.7&0.6&0.0&4.6&0.0&4.8&0.1&513.5&25.9&26.4&5.6\\\hline
		\ref{fn:f19}&330&252&121&0.8&0.0&4.7&0.0&4.7&0.0&407.7&0.5&1.0&0.0&0.8&0.0&4.8&0.0&4.4&0.0&402.9&5.7&1.4&0.8&0.6&0.0&4.6&0.0&4.8&0.1&403.6&0.6&1.0&0.0\\\hline
		\ref{fn:f20}&330&252&121&0.8&0.0&4.7&0.0&4.7&0.0&682.2&145.7&45.2&24.0&0.8&0.0&4.8&0.0&4.5&0.0&607.1&170.8&45.8&28.8&0.8&0.0&4.5&0.0&4.8&0.0&594.1&120.6&46.4&28.3\\\hline
		\ref{fn:f21}&45&42&18&0.6&0.1&2.8&0.7&2.9&0.7&38.4&1.4&1.0&0.0&0.7&0.1&3.0&0.7&2.8&0.6&31.8&1.2&1.0&0.0&0.6&0.1&2.7&0.8&3.0&0.7&33.1&1.5&1.0&0.0\\\hline
		\ref{fn:f22}&45&42&18&0.6&0.1&2.4&0.4&2.5&0.3&38.7&1.1&1.0&0.0&0.6&0.1&2.5&0.4&2.4&0.3&29.4&0.4&1.0&0.0&0.6&0.1&2.3&0.4&2.5&0.4&32.2&1.1&1.0&0.0\\\hline
		
	\end{tabular}
	% 	}
\end{table}

 \begin{table}[htb!]
	% 	\resizebox{\columnwidth}{!}{%
	\tiny
	\centering
	\caption{Total CPU time in seconds taken by rational and polynomial approximation approaches where the interpolation points are selected using \textbf{Sparse Grids}} \label{tab:cputimes3}
	\setlength{\tabcolsep}{2pt}
	\begin{tabular}{|*{34}{c|}} 
		% 			{cc|c|c|c|c|c|c|c|c|c|c|c|c|}
		\cline{5-34}
		\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\multicolumn{10}{|c|}{$\epsilon=0$}
		&\multicolumn{10}{|c|}{$\epsilon=10^{-2}$}
		&\multicolumn{10}{|c|}{$\epsilon=10^{-6}$}
		\\
		\cline{1-34}
		FNo.
		&\makecell{\textit{DoF}\\ for \\poly.\\approx.}
		&\makecell{\textit{DoF}\\ for\\ rational\\approx.}
		&\makecell{\textit{nnl}\\ in \\$q(x)$}
		& \multicolumn{2}{|c|}{\makecell{Poly.\\approx.}}
		& \multicolumn{2}{|c|}{\makecell{Algorithm\\ RA}}
		& \multicolumn{2}{|c|}{\makecell{Algorithm\\ RA with DR}}
		& \multicolumn{4}{|c|}{\makecell{Algorithm\\ ~\ref{A:Polyak}}}
		& \multicolumn{2}{|c|}{\makecell{Poly.\\approx.}}
		& \multicolumn{2}{|c|}{\makecell{Algorithm\\ RA}}
		& \multicolumn{2}{|c|}{\makecell{Algorithm\\ RA with DR}}
		& \multicolumn{4}{|c|}{\makecell{Algorithm\\ ~\ref{A:Polyak}}}
		& \multicolumn{2}{|c|}{\makecell{Poly.\\approx.}}
		& \multicolumn{2}{|c|}{\makecell{Algorithm\\ RA}}
		& \multicolumn{2}{|c|}{\makecell{Algorithm\\ RA with DR}}
		& \multicolumn{4}{|c|}{\makecell{Algorithm\\ ~\ref{A:Polyak}}}
		\\
		\cline{1-34}
		\multicolumn{1}{|c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		& \multicolumn{2}{|c|}{\makecell{iterations}}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		& \multicolumn{2}{|c|}{\makecell{iterations}}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		&\multicolumn{2}{|c|}{time}
		& \multicolumn{2}{|c|}{\makecell{iterations}}
		\\
		\cline{1-34}
		\multicolumn{1}{|c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}&\textit{M}&\textit{SD}
		&\textit{M}&\textit{SD}
		\\
		\hline\hline
		
		\ref{fn:f1}&45&42&18&0.5&0.0&2.0&0.0&2.3&0.0&25.3&0.0&1.0&0.0&0.4&0.0&2.0&0.0&2.2&0.0&21.3&0.0&1.0&0.0&0.4&0.0&2.2&0.0&2.3&0.0&22.1&0.0&1.0&0.0\\\hline
		\ref{fn:f2}&45&42&18&0.4&0.0&2.0&0.0&2.3&0.0&25.3&0.0&1.0&0.0&0.4&0.0&2.0&0.0&2.2&0.0&20.2&0.0&1.0&0.0&0.4&0.0&2.2&0.0&2.3&0.0&22.0&0.0&1.0&0.0\\\hline
		\ref{fn:f3}&45&42&18&0.4&0.0&2.0&0.0&2.3&0.0&23.7&0.0&1.0&0.0&0.4&0.0&2.0&0.0&2.0&0.0&21.0&0.0&1.0&0.0&0.4&0.0&2.2&0.0&2.3&0.0&20.5&0.0&1.0&0.0\\\hline
		\ref{fn:f4}&45&42&18&0.4&0.0&2.0&0.0&2.3&0.0&25.2&0.0&1.0&0.0&0.4&0.0&2.0&0.0&2.0&0.0&23.0&0.0&1.0&0.0&0.4&0.0&2.2&0.0&2.3&0.0&20.9&0.0&1.0&0.0\\\hline
		\ref{fn:f5}&45&42&18&0.4&0.0&2.0&0.0&2.3&0.0&23.9&0.0&1.0&0.0&0.4&0.0&2.0&0.0&2.2&0.0&20.5&0.0&1.0&0.0&0.4&0.0&2.2&0.0&2.3&0.0&20.6&0.0&1.0&0.0\\\hline
		\ref{fn:f7}&45&42&18&0.4&0.0&2.0&0.0&2.3&0.0&24.1&0.0&1.0&0.0&0.4&0.0&2.0&0.0&2.0&0.0&20.5&0.0&1.0&0.0&0.4&0.0&2.2&0.0&2.3&0.0&20.7&0.0&1.0&0.0\\\hline
		\ref{fn:f8}&45&42&18&0.4&0.0&2.0&0.0&2.3&0.0&24.4&0.0&2.0&0.0&0.4&0.0&2.0&0.0&2.0&0.0&21.3&0.0&1.0&0.0&0.4&0.0&2.2&0.0&2.3&0.0&21.7&0.0&1.0&0.0\\\hline
		\ref{fn:f9}&45&42&18&0.4&0.0&2.0&0.0&2.3&0.0&25.4&0.0&1.0&0.0&0.4&0.0&2.0&0.0&2.0&0.0&22.0&0.0&1.0&0.0&0.4&0.0&2.2&0.0&2.3&0.0&22.2&0.0&1.0&0.0\\\hline
		\ref{fn:f10}&330&252&121&0.4&0.0&7.3&0.0&7.9&0.0&504.4&0.0&1.0&0.0&0.4&0.0&6.6&0.0&6.9&0.0&390.1&0.0&1.0&0.0&0.4&0.0&6.8&0.0&7.1&0.0&454.2&0.0&1.0&0.0\\\hline
		\ref{fn:f12}&45&42&18&0.4&0.0&2.0&0.0&2.3&0.0&24.4&0.0&1.0&0.0&0.4&0.0&2.0&0.0&2.2&0.0&20.5&0.0&1.0&0.0&0.4&0.0&2.2&0.0&2.3&0.0&21.1&0.0&1.0&0.0\\\hline
		\ref{fn:f13}&45&42&18&0.4&0.0&2.0&0.0&2.3&0.0&24.0&0.0&1.0&0.0&0.4&0.0&2.0&0.0&2.2&0.0&20.6&0.0&1.0&0.0&0.4&0.0&2.2&0.0&2.3&0.0&20.8&0.0&1.0&0.0\\\hline
		\ref{fn:f14}&45&42&18&0.4&0.0&2.0&0.0&2.3&0.0&25.1&0.0&1.0&0.0&0.4&0.0&2.0&0.0&2.2&0.0&21.6&0.0&1.0&0.0&0.4&0.0&2.2&0.0&2.3&0.0&21.8&0.0&1.0&0.0\\\hline
		\ref{fn:f15}&45&42&18&0.4&0.0&2.0&0.0&2.3&0.0&25.1&0.0&1.0&0.0&0.4&0.0&2.0&0.0&2.2&0.0&20.7&0.0&1.0&0.0&0.4&0.0&2.2&0.0&2.3&0.0&21.8&0.0&1.0&0.0\\\hline
		\ref{fn:f16}&45&42&18&0.5&0.0&2.0&0.0&2.3&0.0&25.2&0.0&1.0&0.0&0.4&0.0&2.0&0.0&2.2&0.0&20.6&0.0&1.0&0.0&0.4&0.0&2.2&0.0&2.3&0.0&21.9&0.0&1.0&0.0\\\hline
		\ref{fn:f17}&120&112&52&0.4&0.0&2.5&0.0&2.7&0.0&54.2&0.0&1.0&0.0&0.4&0.0&2.4&0.0&2.5&0.0&50.9&0.0&1.0&0.0&0.4&0.0&2.6&0.0&2.8&0.0&50.7&0.0&1.0&0.0\\\hline
		\ref{fn:f18}&330&252&121&0.4&0.0&7.3&0.0&7.8&0.0&453.2&0.0&1.0&0.0&-1.0&0.0&-1.0&0.0&-1.0&0.0&-1.0&0.0&-1.0&0.0&-1.0&0.0&-1.0&0.0&-1.0&0.0&-1.0&0.0&-1.0&0.0\\\hline
		\ref{fn:f19}&330&252&121&0.4&0.0&6.2&0.0&7.7&0.0&390.7&0.0&1.0&0.0&0.4&0.0&6.3&0.0&7.0&0.0&394.9&0.0&1.0&0.0&0.4&0.0&6.5&0.0&6.8&0.0&387.5&0.0&1.0&0.0\\\hline
		\ref{fn:f20}&330&252&121&-1.0&0.0&-1.0&0.0&-1.0&0.0&-1.0&0.0&-1.0&0.0&-1.0&0.0&-1.0&0.0&-1.0&0.0&-1.0&0.0&-1.0&0.0&-1.0&0.0&-1.0&0.0&-1.0&0.0&-1.0&0.0&-1.0&0.0\\\hline
		\ref{fn:f21}&45&42&18&0.5&0.0&1.7&0.0&2.0&0.0&23.9&0.0&1.0&0.0&0.4&0.0&1.7&0.0&2.0&0.0&20.0&0.0&1.0&0.0&0.3&0.0&2.0&0.0&2.3&0.0&20.7&0.0&1.0&0.0\\\hline
		\ref{fn:f22}&45&42&18&0.4&0.0&1.7&0.0&1.9&0.0&26.5&0.0&1.0&0.0&0.3&0.0&1.7&0.0&2.0&0.0&20.1&0.0&1.0&0.0&0.3&0.0&1.7&0.0&2.3&0.0&22.6&0.0&1.0&0.0\\\hline
		
	\end{tabular}
	% 	}
\end{table}

\clearpage
%###################################################

%\begin{figure}[htb!]
%	\centering
%	\begin{subfigure}[b]{0.49\textwidth}
%		\centering
%		\includegraphics[width=.8\textwidth]{images/Piterinfo_robarg_f24_p5_q4_ts2x.pdf}
%		\caption{2D \ref{fn:f18} $\epsilon=0$}    
%		\label{fig:f18poles1}
%	\end{subfigure}
%	%	\hfill
%	\begin{subfigure}[b]{0.49\textwidth}  
%		\centering
%		\includegraphics[width=.8\textwidth]{images/Piterinfo_robarg_f24_noisepct10-1_p5_q4_ts2x.pdf}
%		\caption{2D \ref{fn:f18} $\epsilon=10^{-1}$}    
%		\label{fig:f18poles2}
%	\end{subfigure}
%	\vskip\baselineskip
%	\begin{subfigure}[b]{0.49\textwidth}
%		\centering
%		\includegraphics[width=.8\textwidth]{images/Piterinfo_robarg_f23_p5_q4_ts2x.pdf}
%		\caption{3D \ref{fn:f18} $\epsilon=0$}        
%		\label{fig:f18poles3}
%	\end{subfigure}
%	%	\hfill
%	\begin{subfigure}[b]{0.4\textwidth}  
%		\centering
%		\includegraphics[width=.8\textwidth]{images/Piterinfo_robarg_f23_noisepct10-1_p5_q4_ts2x.pdf}
%		\caption{3D \ref{fn:f18} $\epsilon=10^{-1}$}        
%		\label{fig:f18poles4}
%	\end{subfigure}
%	\caption{argmin q(x)}
%	\label{fig:f18poles}
%\end{figure}
%
% \begin{table}[htb!]
%	% 	\resizebox{\columnwidth}{!}{%
%	\small
%	\centering
%	\caption{Getting a better understanding of runtimes and no. of iterations for different dimensions and range of variables for \textit{Sinc} function data} \label{tab:sinctable}
%	\setlength{\tabcolsep}{3pt}
%	\begin{tabular}{|*{7}{c|}} 
%		% 			{cc|c|c|c|c|c|c|c|c|c|c|c|c|}
%		\cline{1-7}
%		\makecell{Dim}
%		&\makecell{\textit{DoF}}
%		&\makecell{\textit{nnl}\\ in \\$q(x)$}
%		& \makecell{l}
%		& \makecell{u}
%		& \makecell{CPU time}
%		& \makecell{Iterations}
%		\\
%		\cline{1-7}
%		\hline\hline
%		2&16&7&$10^{-6}$&$2\pi$&13.991&1\\\hline
%		2&16&7&$10^{-6}$&$4\pi$&15.889&1\\\hline
%		2&16&7&$10^{-3}$&$2\pi$&13.836&2\\\hline
%		2&16&7&$10^{-3}$&$4\pi$&15.836&1\\\hline
%		3&30&16&$10^{-6}$&$2\pi$&16.896&1\\\hline
%		3&30&16&$10^{-6}$&$4\pi$&18.146&9\\\hline
%		3&30&16&$10^{-3}$&$2\pi$&19.978&1\\\hline
%		3&30&16&$10^{-3}$&$4\pi$&17.247&3\\\hline
%		4&50&30&$10^{-6}$&$2\pi$&24.928&2\\\hline
%		4&50&30&$10^{-6}$&$4\pi$&27.053&10\\\hline
%		4&50&30&$10^{-3}$&$2\pi$&24.756&1\\\hline
%		4&50&30&$10^{-3}$&$4\pi$&27.638&14\\\hline
%		5&77&50&$10^{-6}$&$2\pi$&59.864&34\\\hline
%		5&77&50&$10^{-6}$&$4\pi$&77.326&72\\\hline
%		5&77&50&$10^{-3}$&$2\pi$&53.948&21\\\hline
%		5&77&50&$10^{-3}$&$4\pi$&71.326&58\\\hline
%		6&112&77&$10^{-6}$&$2\pi$&125.878&28\\\hline
%		6&112&77&$10^{-6}$&$4\pi$&135.681&39\\\hline
%		6&112&77&$10^{-3}$&$2\pi$&119.904&20\\\hline
%		6&112&77&$10^{-3}$&$4\pi$&195.167&104\\\hline
%		7&156&112&$10^{-6}$&$2\pi$&394.503&61\\\hline
%		7&156&112&$10^{-6}$&$4\pi$&1049.508&381\\\hline
%		7&156&112&$10^{-3}$&$2\pi$&426.752&82\\\hline
%		7&156&112&$10^{-3}$&$4\pi$&841.672&298\\\hline
%	\end{tabular}
%	% 	}
%\end{table}


%%% ========================================================================== %%%
\subsection{Summary of Computational Results}

In this section, we summarize our numerical experiments and observations. 
From our experiments, we conclude that the rational approximation using Algorithm~\ref{ALG:MVVandQR} is a more efficient approach to approximate rational functions when they do not exhibit pole-like behavior. 
However, not all functions we may approximate are rational. 
Also, this approach exhibits pole-like behavior for most  functions, especially when noise is added to the interpolation data, which increases the testing error substantially.
The rational approximation using Algorithm~\ref{A:Polyak} takes more time to remove the poles iteratively, but the final approximation is largely devoid of poles, which is particularly significant for noisy interpolation data. 
Additionally, the quality of the approximation with this approach is better than the other two approaches in both the noise-fee and noisy cases. 
As we will see in the next section, the additional time to get a pole-free and a superior quality of approximation is small price to pay considering that this approximation replaces expensive simulations of the physics processes.




==> numerics-old2.tex <==
\section{Old Numerical Results}

\sven{ToDo: Start here with the numerical experiments, and try the two approaches from the previous section; make sure the examples have no poles in $[l,u]$!}
We have created three test problems in 2D of increasing difficulty over $\p = (x_1,x_2)$ to test our
formulation (and it kind of works):
\begin{eqnarray}
  f_1(x_1,x_2) & = & \dps \frac{x_1^2 + 2x_1x_2 + x_2^2 +1}{1+x_1-x_2} \\
  f_2(x_1,x_2) & = & \dps \frac{\exp(x_1 + 2x_2) -x_1 + x_2 -1}{1+2x_1+x_2} \\
  f_3(x_1,x_2) & = & \dps \frac{\exp(x_1 + 2x_2) -x_1 - 2x_2 +1}{1 + \log(x_1+x_2+1)}
\end{eqnarray}
which are defined over $[-1,1]^2$.
\sven{Look at Anthony's test problems, see {\tt testcases.mat}!}

For our experiments, we first randomly generate 9 points in  $[-1,1]^2$ (which should uniquely
determine the 9 coefficients ... it does not, of course!). We then solve a version of the
interpolation problem
(using AMPL), and then generate a random $20 \times 20$ grid in $[-1,1]^2$ on which we
compute the difference between $f_i$ and its rational approximation. We also use the same
interpolation points to fit a cubic (which in 2D is uniquely determined by 9 (random!) points),
and again compute the difference. Figures~\ref{fig:PadeRes1}-\ref{fig:PadeRes3} plot the error
over  $[-1,1]^2$ (in each case the left figure is the rational and the right the cubic
approximation. Not surprisingly, the rational does better. Interestingly, the error of the
rational is largest close to the singularity.

\paragraph{Open Questions}
\begin{enumerate}
  \item Compare to other forms of interpolants.
  \item Can we prove convergence within a trust-region framework?
  \item Apply to an interesting physics problem \& show its better!
  \item Theory of interpolation: well-posedness, uniqueness, scaling?
\end{enumerate}


\begin{figure}[htb]
  \begin{center}
    \includegraphics[width=0.45\textwidth]{PadeLogApproxError1}\hfill
    \includegraphics[width=0.45\textwidth]{CubicLogApproxError1}
    \caption{Logarithm of approximation error for rational (left) and cubic (right)
      for function $f_1(x_1,x_2)$.}\label{fig:PadeRes1}
  \end{center}
\end{figure}
\begin{figure}[htb]
  \begin{center}
    \includegraphics[width=0.45\textwidth]{PadeLogApproxError2}\hfill
    \includegraphics[width=0.45\textwidth]{CubicLogApproxError2}
    \caption{Logarithm of approximation error for rational (left) and cubic (right)
      for function $f_2(x_1,x_2)$.}\label{fig:PadeRes2}
  \end{center}
\end{figure}
\begin{figure}[htb]
  \begin{center}
    \includegraphics[width=0.45\textwidth]{PadeLogApproxError3}\hfill
    \includegraphics[width=0.45\textwidth]{CubicLogApproxError3}
    \caption{Logarithm of approximation error for rational (left) and cubic (right)
      for function $f_3(x_1,x_2)$.}\label{fig:PadeRes3}
  \end{center}
\end{figure}


==> optimalDegreeData.tex <==
\section{Description of the Polynomial Orders}\label{SEC:DegData}

In this appendix, we describe the polynomial orders that were observed on the Pareto front when we ran Algorithm~\ref{A:optdegree} on the interpolation data for several functions in Table~\ref{T:TPs}. Additionally, this appendix also reports the orders that were found to be optimal using our approach and the ones with lowest testing error . These orders are described for non-noisy data in Table~\ref{tab:degData0noise} and for noisy data in Tables~\ref{tab:degData10-6noise}, \ref{tab:degData10-3noise}, and \ref{tab:degData10-1noise} where the amount of noise is described using $\epsilon$ from \eqref{eq:noise}. 

\begin{table}[htb!]
	\caption{Observed polynomial orders with no noise in the training data} \label{tab:degData0noise}
	%	\resizebox{\columnwidth}{!}{%
	\centering
	\begin{tabular}{|c|c|c|c|c|}
		\cline{1-5}
		\cline{1-5}
		\makecell{Function \\No.} &
		\makecell{Polynomial order on Pareto \\ front in ascending order\\ of the $\log_{10}(\eta_{MN})$} &
		\makecell{Actual Order \\from\\Table~\ref{T:TPs}}&
		\makecell{Optimal Order \\obtained from \\Algorithm~\ref{A:optdegree}}&
		\makecell{Order with \\lowest $\Delta_{MN}$}
		\\
		\cline{1-5}
		\ref{fn:f1}&\makecell{(2, 0), (1, 2), (2, 2), (4, 2), (3, 4),\\(4, 4), (2, 6), (4, 6), (5, 6), (4, 7),\\(6, 6), (7, 6)}&(-,4)&(2,6)&(7, 6)\\\hline
		\ref{fn:f4}&(2, 0), (2, 1), (3, 0), (2, 2), (4, 4)&(-,-)&(2,2)&(4, 4)\\\hline
		\ref{fn:f7}&\makecell{(2, 0), (2, 1), (3, 0), (2, 2), (3, 1),\\(4, 0), (3, 2), (3, 3)}&(3,3)&(3,3)&(3, 3)\\\hline
		\ref{fn:f8}&\makecell{(1, 1), (1, 2), (2, 2), (2, 3), (3, 3),\\(2, 4), (3, 4)}&(2,2)&(2,3)&(3, 4)\\\hline
		\ref{fn:f9}&\makecell{(2, 0), (1, 2), (2, 2), (4, 2), (4, 4),\\(5, 4), (6, 4), (6, 5)}&(4,4)&(4,4)&(6, 5)\\\hline
		\ref{fn:f12}&(2, 0), (2, 1), (2, 2), (2, 3)&(2,3)&(2,3)&(2, 3)\\\hline
		\ref{fn:f13}&(1, 1), (1, 2), (3, 0), (3, 1), (3, 2)&(3,2)&(3,2)&(3, 2)\\\hline
		\ref{fn:f14}&(2, 0), (1, 2), (2, 2), (4, 2), (4, 4)&(4,4)&(4,4)&(4, 4)\\\hline
		\ref{fn:f15}&\makecell{(1, 1), (1, 2), (3, 0), (3, 2), (3, 4),\\(5, 6)}&(3,4)&(3,4)&(5, 6)\\\hline
		\ref{fn:f16}&\makecell{(2, 0), (2, 1), (2, 2), (4, 1), (4, 2),\\(4, 3), (5, 5)}&(4,3)&(4,3)&(5, 5)\\\hline
		\ref{fn:f22}&(2, 0), (2, 1)&(2,0)&(2,1)&(2, 1)\\\hline
		
		% \hline
		% \multicolumn{1}{|c|}{astar} & & * &  & * &  &  & * &\\
		\hline
	\end{tabular}
	%	}
\end{table}

\begin{table}[htb!]
	\caption{Observed polynomial orders with noise in the training data described using $\epsilon=10^{-6}$} \label{tab:degData10-6noise}
	%	\resizebox{\columnwidth}{!}{%
	\centering
	\begin{tabular}{|c|c|c|c|c|}
		\cline{1-5}
		\cline{1-5}
		\makecell{Function \\No.} &
		\makecell{Polynomial order on Pareto \\ front in ascending order\\ of the $\log_{10}(\eta_{MN})$} &
		\makecell{Actual Order \\from\\Table~\ref{T:TPs}}&
		\makecell{Optimal Order \\obtained from \\Algorithm~\ref{A:optdegree}}&
		\makecell{Order with \\lowest $\Delta_{MN}$}
		\\
		\cline{1-5}
		\ref{fn:f1}&\makecell{(2, 0), (1, 2), (2, 2), (4, 2), (3, 4),\\(4, 4), (2, 6), (4, 6), (5, 6), (4, 7),\\(6, 6), (7, 6), (7, 7)}&(-,4)&(4,6)&(7, 7)\\\hline
		\ref{fn:f4}&(2, 0)&(-,-)&(2,0)&(2, 0)\\\hline
		\ref{fn:f7}&\makecell{(2, 0), (2, 1), (3, 0), (2, 2), (3, 1),\\(4, 0), (3, 2), (3, 3), (3, 5)}&(3,3)&(3,3)&(3, 5)\\\hline
		\ref{fn:f8}&(1, 1), (1, 2), (2, 2), (2, 3), (3, 3)&(2,2)&(2,2)&(3, 3)\\\hline
		\ref{fn:f9}&(2, 0), (1, 2), (2, 2), (4, 2), (4, 4)&(4,4)&(4,4)&(4, 4)\\\hline
		\ref{fn:f12}&(2, 0), (2, 1), (2, 2), (2, 3)&(2,3)&(2,3)&(2, 3)\\\hline
		\ref{fn:f13}&\makecell{(1, 1), (1, 2), (3, 0), (3, 1), (3, 2),\\(4, 3)}&(3,2)&(3,0)&(4, 3)\\\hline
		\ref{fn:f14}&(2, 0), (1, 2), (2, 2), (4, 2), (4, 4)&(4,4)&(4,4)&(4, 4)\\\hline
		\ref{fn:f15}&\makecell{(1, 1), (1, 2), (3, 0), (3, 2), (3, 4),\\(3, 6)}&(3,4)&(3,4)&(3, 6)\\\hline
		\ref{fn:f16}&\makecell{(2, 0), (2, 1), (2, 2), (4, 1), (4, 2),\\(4, 3), (5, 3), (6, 3)}&(4,3)&(5,3)&(6, 3)\\\hline
		\ref{fn:f22}&(2, 0), (2, 1)&(2,0)&(2,1)&(2, 1)\\\hline
		
		% \hline
		% \multicolumn{1}{|c|}{astar} & & * &  & * &  &  & * &\\
		\hline
	\end{tabular}
	%	}
\end{table}

\begin{table}[htb!]
	\caption{Observed polynomial orders with noise in the training data described using $\epsilon=10^{-3}$} \label{tab:degData10-3noise}
	%	\resizebox{\columnwidth}{!}{%
	\centering
	\begin{tabular}{|c|c|c|c|c|}
		\cline{1-5}
		\cline{1-5}
		\makecell{Function \\No.} &
		\makecell{Polynomial order on Pareto \\ front in ascending order\\ of the $\log_{10}(\eta_{MN})$} &
		\makecell{Actual Order \\from\\Table~\ref{T:TPs}}&
		\makecell{Optimal Order \\obtained from \\Algorithm~\ref{A:optdegree}}&
		\makecell{Order with \\lowest $\Delta_{MN}$}
		\\
		\cline{1-5}
		\ref{fn:f1}&\makecell{(2, 0), (1, 2), (2, 2), (4, 2), (3, 4),\\(4, 4), (2, 6)}&(-,4)&(2,2)&(2, 6)\\\hline
		\ref{fn:f4}&(2, 0), (2, 1), (3, 3)&(-,-)&(2,1)&(3, 3)\\\hline
		\ref{fn:f7}&\makecell{(2, 0), (2, 1), (3, 0), (2, 2), (3, 1),\\(4, 0), (3, 2), (3, 3), (4, 3), (4, 4),\\(6, 1), (6, 2), (6, 3)}&(3,3)&(3,0)&(6, 3)\\\hline
		\ref{fn:f8}&(1, 1), (1, 2), (2, 2), (2, 3), (3, 3)&(2,2)&(2,2)&(3, 3)\\\hline
		\ref{fn:f9}&\makecell{(2, 0), (1, 2), (2, 2), (4, 2), (4, 4),\\(5, 4), (6, 4)}&(4,4)&(2,2)&(6, 4)\\\hline
		\ref{fn:f12}&(2, 0), (2, 1), (2, 2), (2, 3)&(2,3)&(2,3)&(2, 3)\\\hline
		\ref{fn:f13}&\makecell{(1, 1), (1, 2), (3, 0), (3, 1), (3, 2),\\(3, 3)}&(3,2)&(3,0)&(3, 3)\\\hline
		\ref{fn:f14}&\makecell{(2, 0), (1, 2), (2, 2), (4, 2), (5, 2),\\(4, 4)}&(4,4)&(2,2)&(4, 4)\\\hline
		\ref{fn:f15}&(1, 1), (1, 2), (3, 0), (3, 2), (3, 4)&(3,4)&(3,4)&(3, 4)\\\hline
		\ref{fn:f16}&\makecell{(2, 0), (2, 1), (2, 2), (4, 1), (4, 2),\\(4, 3), (5, 4)}&(4,3)&(4,1)&(5, 4)\\\hline
		\ref{fn:f22}&(2, 0), (2, 1)&(2,0)&(2,1)&(2, 1)\\\hline
		
		% \hline
		% \multicolumn{1}{|c|}{astar} & & * &  & * &  &  & * &\\
		\hline
	\end{tabular}
	%	}
\end{table}

\begin{table}[htb!]
	\caption{Observed polynomial orders with noise in the training data described using $\epsilon=10^{-1}$} \label{tab:degData10-1noise}
	%	\resizebox{\columnwidth}{!}{%
	\centering
	\begin{tabular}{|c|c|c|c|c|}
		\cline{1-5}
		\cline{1-5}
		\makecell{Function \\No.} &
		\makecell{Polynomial order on Pareto \\ front in ascending order\\ of the $\log_{10}(\eta_{MN})$} &
		\makecell{Actual Order \\from\\Table~\ref{T:TPs}}&
		\makecell{Optimal Order \\obtained from \\Algorithm~\ref{A:optdegree}}&
		\makecell{Order with \\lowest $\Delta_{MN}$}
		\\
		\cline{1-5}
		\ref{fn:f1}&(2, 0), (1, 2), (2, 2), (4, 2)&(-,4)&(1,2)&(4, 2)\\\hline
		\ref{fn:f4}&(1, 1), (1, 2), (3, 3)&(-,-)&(1,2)&(3, 3)\\\hline
		\ref{fn:f7}&(2, 0), (2, 1), (2, 2), (5, 7)&(3,3)&(2,2)&(5, 7)\\\hline
		\ref{fn:f8}&(1, 1), (1, 2), (2, 2), (3, 2), (3, 3)&(2,2)&(3,2)&(3, 3)\\\hline
		\ref{fn:f9}&\makecell{(2, 0), (1, 2), (2, 2), (2, 4), (4, 4),\\(6, 2)}&(4,4)&(4,4)&(6, 2)\\\hline
		\ref{fn:f12}&\makecell{(2, 0), (2, 1), (2, 2), (3, 1), (3, 2),\\(3, 3)}&(2,3)&(3,1)&(3, 3)\\\hline
		\ref{fn:f13}&\makecell{(1, 1), (1, 2), (3, 0), (3, 1), (3, 2),\\(3, 3), (5, 1)}&(3,2)&(3,3)&(5, 1)\\\hline
		\ref{fn:f14}&(2, 0), (1, 2), (2, 2), (4, 2), (4, 3)&(4,4)&(4,2)&(4, 3)\\\hline
		\ref{fn:f15}&(1, 1), (1, 2), (3, 0), (3, 2), (4, 2)&(3,4)&(3,0)&(4, 2)\\\hline
		\ref{fn:f16}&\makecell{(2, 0), (2, 1), (2, 2), (4, 2), (4, 3),\\(4, 4)}&(4,3)&(2,1)&(4, 4)\\\hline
		\ref{fn:f22}&(2, 0), (2, 1), (3, 3)&(2,0)&(2,1)&(3, 3)\\\hline
		
		% \hline
		% \multicolumn{1}{|c|}{astar} & & * &  & * &  &  & * &\\
		\hline
	\end{tabular}
	%	}
\end{table}

==> plans.tex <==
\section{Plans for Possible Papers}\label{sec:plans}

\begin{enumerate}
  \item {\bf Comparison on Simple Test Problems.} Create some simple test problems like the ones
    above, and compute the rational approximation.
  \item {\bf Comparison of Static Tunes.} Generate polynomial and rational
    approximations, and compare them. Properties of interest include (1) ease of computation,
    (2) robustness, (3) local approximation properties, (4) global approximation properties.
    We would need to develop a plan on how to compare and evaluate the tunes.
\end{enumerate}
  


==> pyrapp.tex <==
%\section{\textcolor{blue}{take out and put into other paper?}Choosing the Degree of the Polynomials}\label{SEC:degree}

%In the previous sections we have described two approaches for computing the rational approximations, assuming that the polynomial orders of the numerator and the denominator are given. However, in practice these orders might be a priori unknown. Thus, we describe and evaluate a heuristic for selecting the ``optimal'' order of the numerator and denominator polynomials. We  build on information-theoretic approaches and a multi-objective perspective that balances the number of coefficients and the testing error. 
%\sven{A possible section outline is:}

%\begin{enumerate}
%  \item Describe the approach we take in general ... view as outer loop of rational approximation.
%  \item Justify/motivate the approach using stats?
%  \item Compare the approach to a simple approach ...
%  \item Show how the approach works for noise-free data and for different amounts of noise.
%  \item Conclusions/summary of our experience.
%\end{enumerate}

%\subsection{A heuristic algorithm for selecting the optimal order of the polynomials}
%Our heuristic  algorithm first finds  the  Pareto optimal solutions  
%that minimize both the  testing error $\Delta_r$ and the number of coefficients $\eta_r$ of the rational approximations $r\in\mathcal{R}$.
%We select one Pareto optimal solution that determines  the ``optimal'' polynomial orders using  the triangle method for finding the corner of the L-curve (see \cite{CASTELLANOS2002359}). Keeping $C$ fixed at the rightmost point of the Pareto front i.e., the point with the highest $x$ coordinate, vertices $A$ and $B$ are moved from left to the right such that $B$ occurs before $A$ on the $x$ coordinate \textcolor{blue}{this $x$ denotes an axis in the objective space? this is different from our parameters $x$, right?}. 
%On the front, the triangle \textit{BAC} may either form an L or an inverted-L as shown in Figure~\ref{fig:TrBAC}. 
%The (signed) area $\mathcal{A}$ of triangle \textit{BAC} can be computed as
%\begin{equation}\label{EQN:area}
%\mathcal{A}(BAC)= \frac{1}{2}~\\\mathrm{det}\begin{vmatrix} x^{(B)} & y^{(B)} & 1 \\ x^{(A)} & y^{(A)} &1\\x^{(C)} & y^{(C)} &1 \end{vmatrix}
%\end{equation}
%where the determinant is positive if \textit{BAC} is listed in counterclockwise order and therefore shaped as an L and it is negative if \textit{BAC} is listed in clockwise order or shaped as an inverted-L~\cite{zwillinger2018crc}. Hence, a triangle \textit{BAC} with a positive $\mathcal{A}$ that has the largest angle at $A$ $\ge \frac{7\pi}{2}$ is chosen as the corner \textcolor{blue}{A is chosen as corner?}. If no such corner can be found, then $C$ is chosen as the corner. The order of polynomials corresponding to the chosen corner is then the optimal order of the polynomials. \textcolor{blue}{worthwhile defining the multi-objective problem in parameters $m$ and $n$ (degrees of nominator and denominator)? or more illustrative image of this corner-process on a Pareto front image?}
%The pseudocode of our method is shown in  Algorithm~\ref{A:optdegree}.

%\begin{figure}[htb!]
%	\centering
%\begin{tikzpicture}\label{dsds}
%\draw (0,3) node[anchor=south]{$B (x^{(B)},y^{(B)})$}
%-- (1,0) node[anchor=north]{$A (x^{(A)},y^{(A)})$}
%-- (6,-1) node[anchor=north]{$C (x^{(C)},y^{(C)})$}

%-- cycle;
%\draw (7,3) node[anchor=south]{$B (x^{(B)},y^{(B)})$}
%-- (11,2.5) node[anchor=south]{$A (x^{(A)},y^{(A)})$}
%-- (13,-1) node[anchor=north]{$C (x^{(C)},y^{(C)})$}

%-- cycle;
%\end{tikzpicture}
%\caption{Triangle \textit{BAC} shaped as an L when viewed counterclockwise (left) and as an inverted-L when viewed clockwise (right)} \label{fig:TrBAC}
%\end{figure}


%\begin{algorithm2e}[htb!]
%	\DontPrintSemicolon \setcounter{AlgoLine}{0}
%	\caption{Choosing the polynomial order of the approximation}\label{A:optdegree}
%	\SetKwInOut{Input}{Input}
%	\SetKwInOut{Output}{Output}
%	\Input{$\mathcal{M}$ and $\mathcal{N}$, which are the ranges for the orders of the numerator and denominator polynomial, respectively, a set $\mathcal{R}$ of approximations obtained using \eqref{eq:rofxopts} for orders $M\in\mathcal{M}$ and $N\in\mathcal{N}$.}
%	\Output{$M^{(corner)}, N^{(corner)}$ associated with $\hat{P}^{(corner)}$.}
%	Let $\mathcal{M}$ and $\mathcal{N}$ be the ranges for the numerator and denominator polynomial degrees, respectively\;
%	Let $\mathcal{R}$ be the set of approximations obtained using \eqref{eq:rofxopts} for $\mathcal{M}$ and $\mathcal{N}$\;
%	using Algorithms~\ref{ALG:MVVandQR},~\ref{A:Polyak}, or polynomial approximation with $N\gets0$\;
%	Let $\Delta_r$ be the testing error for $r \in \mathcal{R}$ calculated using \eqref{eq:testError}\;
%	Let $\eta_r \gets \alpha(M) + \alpha(N)$ be the number of coefficients for each $r \in \mathcal{R}$\;
%	Let $P \gets \{(log_{10}(\eta_r),log_{10}(\Delta_r))~|~r \in \mathcal{R}\}$\;
%	Let $\hat{P}^{(1)},\dots,\hat{P}^{(n)}$ be the Pareto front for $P$, sorted in ascending order of $log_{10}(\eta_r)$\;
%	$\theta_{max} \gets -2,$ corner$ \gets n, C \gets \hat{P}^{(n)}$\;
%	\For{$i \gets 1$ to $n-2$}{
%		$B \gets \hat{P}^{(i)}$\;
%		\For{$j \gets i$ to $n-2$}{
%			$A \gets \hat{P}^{(j+1)}$\;
%			Compute $\mathcal{A}(\mathrm{\textit{BAC}})$ using \eqref{EQN:area}\;
%			$\theta_A \gets \cos^{-1}\left(\frac{\overline{AB}\cdot\overline{AC}}{||\overline{AB}||~||\overline{AC}||}\right)$\;
%			\If{$\theta_A\ge7\pi/2$ and $\theta_A\ge\theta_{max}$ and $\mathcal{A}(\mathrm{\textit{BAC}})>0$}{
%				corner $\gets j+1$\;
%				$\theta_{max} \gets \theta_A$\;
%			}
%		}
%	}
%	\Return{$M^{(corner)}, N^{(corner)}$ associated with $\hat{P}^{(corner)}$}
%\end{algorithm2e}

%\begin{figure}[htb!]
%	\centering
%	\resizebox{\textwidth}{4in}{
%		\input{images/Poptdegcomparesubplots.pgf}
%	}
%	\caption{Plots of test metric vs the degrees of freedom of different approximation orders for functions in Table~\ref{T:TPs}. The red and blue circles are the rational and polynomial approximation orders on the Pareto front, respectively. The star is the optimal order chosen by Algorithm~\ref{A:optdegree} and the \textit{purple X} is the order with the lowest test error}
%	\label{fig:optdegcomparisonplots}
%\end{figure}



%\subsection{Motivating examples and comparison to a naive approach}

%In this section, we motivate the use of Algorithm~\ref{A:optdegree} to select the optimal order of the numerator and denominator polynomials by showing plots of how our approach performs compared to a naive approach of selecting orders by only minimizing the  testing error. 
%Figure~\ref{fig:optdegcomparisonplots} shows these plots for four functions from Table~\ref{T:TPs}. The Pareto front, which is shown as red and blue circles for rational and polynomial approximation orders, respectively find the orders that optimize the multiple objectives of minimizing the testing error and the number of degrees of freedom of the approximation. 
%To then find the optimal order from the Pareto front, our approach builds on information-theoretic approaches of AKAIKE's information criterion that deals with a trade-off between the goodness of fit of the model and the number of parameters required to describe the interpolation data~\cite{Akaike1998}.
%Hence, the chosen optimal order that is shown in the plots using a star is the corner of the L on the Pareto front that not only minimizes the testing error, but does this with the minimum number of degrees of freedom required to describe the interpolation data succinctly. 

%The order of the polynomials of the approximations that are on the Pareto front in Figure~\ref{fig:optdegcomparisonplots} is listed in Table~\ref{tab:degData0noise}.
%The optimal orders of the numerator and denominator polynomials selected by our algorithm for functions~\ref{fn:f1}, \ref{fn:f4}, \ref{fn:f8}, and \ref{fn:f14} is (2,6), (2,2), (2,3), and (4,4), respectively. 
%In the original function, both non-rational functions~\ref{fn:f1} and~\ref{fn:f4} have similarly ordered exponential functions in the numerator. But function~\ref{fn:f1} has a fourth order polynomial in the denominator. It is interesting that the optimal degree for the denominator polynomial chosen by our algorithm for function~\ref{fn:f1} is four more than that of function~\ref{fn:f4}. 
%For rational function~\ref{fn:f14}, our approach finds the exact order of the numerator and denominator polynomial as in the original function. 
%In function~\ref{fn:f8}, our approach selects a very close neighbor to the right of exact degree of the original function on the Pareto front. 
%A naive approach of selecting the orders of the polynomials is the one with the lowest testing error as shown in Figure~\ref{fig:optdegcomparisonplots} using \textit{purple X}. Out of the plots for four functions, the naive approach works only for function~\ref{fn:f14}. However, this is a lucky coincidence since the testing error will decrease further if even higher orders of polynomials are chosen to do the approximation. Hence, the naive approach ends up over fitting to the data and our approach suggests more suitable orders of polynomials of the approximation than the naive approach. 


%\subsection{Comparison of optimal polynomial degrees obtained for approximations trained with noise-free and noisy data}

%\begin{figure}[htb!]
%	\centering
%	\resizebox{\textwidth}{4in}{
%		\input{images/Poptdegcomparebarplots.pgf}
%	}
%	\caption{Polynomial orders obtained when the approximations are trained with noise-free and noisy data where the amount of noise is described using $\epsilon$ from \eqref{eq:noise}}
%	\label{fig:optdegcomparisonbarplots}
%\end{figure}
%In the previous subsection, the orders of the polynomials were chosen for functions whose rational and polynomial approximations were trained over noise-free data. In this subsection, we compare the orders chosen by our approach when the approximations are trained using noise-free and noisy data. In particular, we compare the polynomial orders obtained for 2D rational and polynomial functions in Table~\ref{T:TPs} with the actual degree of the polynomials. The rational approximation was performed using Algorithm~\ref{A:Polyak}.
%The results are summarized in Figure~\ref{fig:optdegcomparisonbarplots}. The orders of the polynomials obtained for each case is listed in Tables~\ref{tab:degData0noise},~\ref{tab:degData10-6noise},~\ref{tab:degData10-3noise}, and~\ref{tab:degData10-1noise}. It can be observed that of the nine functions considered, we recover the actual degrees of the polynomials for seven functions when the training data has no noise and for six functions when the noise added to training data is of the order of $\epsilon=10^{-6}$. 
%However, it should be noted that for the functions where the actual degree of the polynomials is not recovered in the cases above, this degree is on the Pareto front and they are either the left or right neighbor of the degree selected. 
%Additionally, for higher levels of noise, the approximations have to contend with larger perturbations and more spurious poles, thereby requiring polynomial orders other than the actual one to fit well to the interpolation data.  

%From the comparison plots above, we conclude that Algorithm~\ref{A:optdegree} provides a good heuristic for selecting the optimal order of numerator and denominator polynomials. In particular, the results above show that the Pareto front filters the polynomial orders that minimize the testing error and the degrees of freedom of the approximation. 
%With no noise or very little noise, the actual order of the polynomials is always on the Pareto front. 
%Additionally, the corner finding method over the front filters the neighborhood within which the optimal order can be found. In fact, our experiments above show that the optimal order is either the selected degree or one of its neighbors on the front. This further reduces the polynomial orders that could be a potential good fit to the interpolation data.







%
%\sven{Work the remainder into this section ...}
%We generate 2-dimensional test data by randomly sampling $N_\text{test}=300$
%points $P$ from the interval $[0,10]\otimes[0,10]$ and evaluating
%\eqref{eq:2dtestdata} to obtain the vector of function values $\vec{F}$.
%
%\begin{equation}\label{eq:2dtestdata}
%    f(x,y) = \frac{10x^2 - y^3 + xy^2}{x^5 -y^2 -4x +5y + 201}
%\end{equation}
%
%We construct the rational approximations $r_{mn}$ for all combinations $m,n \in [0,9]$.
%
%For those, we calculate the ``residual'' difference $\Delta_{mn}$:
%
%\begin{equation}\label{eq:residual}
%    \Delta_{mn} = \frac{\sum\limits_{p,f \in P, \vec{F}} \left|\frac{  r_{mn}(p) - f}{f} \right|}{N_\text{test}}
%\end{equation}
%
%For each $r_{mn}$ we numerically minimize the absolute value of the denominator
%polynomial in the interpolation domain with the L-BFGS-B algorithm and compare
%the found minimum value with a threshold value of $10^{-6}$ in order to
%conservatively guard us against spurious poles in $r_{mn}$.
%
%We consider the best solution to be the one which yields the smallest $\Delta_{mn}$
%and does not have a root in the denominator.
%
%In Fig. \ref{fig:residuals2d}, the residuals are shown in color coding for all
%$m,n$ considered.  Those $r_{mn}$ with a root in the denominator are marked
%with a red x.
%
%\begin{figure}[h]
%    \centering
%    \includegraphics[width=.5\textwidth]{images/2dresidual_mn.pdf}
%    \caption{Approximation error for 2-dimensional test data. In color coding
%        we find the residual measure as defined in \eqref{eq:residual}. The red
%        crosses indicate those $r_{mn}$ where the absolute value of the
%        numerically determined minimum of the denominator polynomial in the
%        interpolation domain is smaller than $10^{-6}$. The best solution is
%        indicated with a star shaped marker.}
%    \label{fig:residuals2d}
%\end{figure}


==> studies-sm.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Studies}

\begin{verbatim}
def coeffSolve2(self, VM, VN):
        """
        This does the solving for the numerator and denominator coefficients
        following Steve's recipe.
        """
        Feps = - (VN.T * self._Y).T
        # the full left side of the equation
        y = np.hstack([ VM, Feps[:,1:self._Y.size ] ])
        U, S, V = np.linalg.svd(y)
        # manipulations to solve for the coefficients
        # Given A = U Sigma VT, for A x = b, x = V Sigma^-1 UT b
        tmp1 = np.transpose( U ).dot( np.transpose( self._Y ))[0:S.size]
        Sinv = np.linalg.inv( np.diag(S) )
        x = np.transpose(V).dot( Sinv.dot(tmp1) )
        self._acoeff = x[0:self._M]
        self._bcoeff = np.concatenate([np.array([1.00]),x[self._M:self._M+self._N+1]])


\end{verbatim}

Define the rational polynomial approximation to $f(x)$ as $f(x) = p_M(x)/q_N(x)$ with $p_M(x) = a_0
+ a_1 x + \cdots + a_M x^M$ and $q_N(x) = 1 + b_1 x + \cdots + b_N
x^N$.
Note, in particular, that $b_0 \equiv 1$.
$f(x)$ is known at $K$ values of $x$ such that $f(x_i) \equiv f_i,
i=1,K$.   At any given point $x_i$, the coefficients of the
polynomials are constrained by the equation:
\begin{eqnarray*}
\begin{matrix}
p_M(x_i) - f(x_i) q_N(x_i) = 0 \\ 
a_0 + a_1 x_i + \cdots + a_M x_i^M - b_1 f_i  x_i - \cdots - b_N f_i x_i^N = f_i
\end{matrix}
\end{eqnarray*}
This manipulation is only possible if $b_0 \equiv 1$.

For $K$ such constraints, we have the matrix representation:

\newcommand{\MyMat}[3]{
                \begin{matrix}
                   \phantom{-}1 &  #1_1 & \cdots    & #1_1^{#2}\\ 
                   \phantom{-}1 & \cdots & \cdots   & \cdots\\
                   \phantom{-}1 &  #1_{#3} & \cdots & #1_{#3}^{#2} 
                \end{matrix}
}

\newcommand{\MyMatM}[3]{
                \begin{matrix}
                   -1 &  #1_1 & \cdots    & #1_1^{#2}\\ 
                   -1 & \cdots & \cdots   & \cdots\\
                   -1 &  #1_{#3} & \cdots & #1_{#3}^{#2} 
                \end{matrix}
}


\newcommand{\FMat}[4]{
                \begin{matrix}
                   #4_1 #1_1 & \cdots    & #4_1 #1_1^{#2}\\ 
                   \cdots & \cdots   & \cdots\\
                   #4_{#3} #1_{#3} & \cdots & #4_{#3} #1_{#3}^{#2} 
                \end{matrix}
}
\newcommand{\ColMat}{
a_0 \\
\cdots \\
a_M \\
b_1 \\
\cdots \\
b_N
}
\newcommand{\FColMat}{
f_1 \\
\cdots \\
\cdots \\
f_K
}

\newcommand{\spaceM}[1]{
\begin{matrix}
 \phantom{#1} \\
 \; \\
 \; \\ 
\end{matrix}
}


\begin{eqnarray*}
&
\begin{bmatrix}
\MyMat{x}{M}{K} \spaceM{1} 
\FMat{x}{N}{K}{-f}
\end{bmatrix}
\begin{bmatrix}
\ColMat
\end{bmatrix} 
= 
\begin{bmatrix}
\FColMat
\end{bmatrix} 
&\\
&\mathrm{or} &\\
&
\begin{bmatrix}
\bf M
\end{bmatrix}
\begin{bmatrix}
z
\end{bmatrix}
=
\begin{bmatrix}
c
\end{bmatrix}
&
\end{eqnarray*}

In particular, we are interested in those cases when $K > M + N$,
{\it{i.e.}} the problem is overconstrained.
%Our problem is in the form $ A x = b$, where $A$ is the matrix in the
%left of our equation, $x$ represents the coefficients of the
%polynomials, and $b$ represents the function values.   
An SVD decomposition of {\bf M}, given $c$, allows for a solution
of the coefficients $z$:
\begin{eqnarray*}
\begin{matrix}
M = U \Sigma V^T \\
z = V^T ( \Sigma^{-1} U^{T} c )\\
a_0 = z[0], a_1 = z[1], \cdots, a_M = z[M], b_0 = 1, b_1 = z[M+1], \cdots, b_N
= z[M+N]
\end{matrix}
\end{eqnarray*}

Our problem is ultimately one of minimization to
find the optimal polynomial coefficients given the constraints, which
are noisy in practice.    An alternative approach is to add the noise
from the start by shifting the function values $f_i$ by
$\pm\epsilon$ with the values $f_i^{\pm}$.    The constraints on the
coefficients are now doubled to $p(x_i)/q(x_i) < f_i^{+}$, and $f_i^{-}
< p(x_i)/q(x_i)$. 



\renewcommand{\FColMat}[1]{
#1_1 \\
\cdots \\
\cdots \\
#1_K
}



\begin{eqnarray*}
\begin{bmatrix}
\MyMat{\phantom{-}x}{M}{K} \spaceM{1} \FMat{x}{N}{K}{-f^{+}} \\ 
\MyMatM{-x}{M}{K} \spaceM{1} \FMat{x}{N}{K}{\phantom{-}f^{-}}
\end{bmatrix} 
\begin{bmatrix}
\ColMat
\end{bmatrix}
<
\begin{bmatrix}
\FColMat{\phantom{-}b_0f^+} \\
\FColMat{-b_0f^-}
\end{bmatrix}
\end{eqnarray*}

This constraints problem is amenable to a  minimization
of the sum of squares of coefficients.


